Large-Scale Secure XGB for Vertical Federated Learning

Privacy-preserving machine learning has drawn increasingly attention recently, especially with kinds of privacy regulations come into force. Under such situation, Federated Learning (FL) appears to facilitate privacy-preserving joint modeling among multiple parties. Although many federated algorithms have been extensively studied, there is still a lack of secure and practical gradient tree boosting models (e.g., XGB) in literature. In this paper, we aim to build large-scale secure XGB under vertically federated learning setting. We guarantee data privacy from three aspects. Specifically, (i) we employ secure multi-party computation techniques to avoid leaking intermediate information during training, (ii) we store the output model in a distributed manner in order to minimize information release, and (iii) we provide a novel algorithm for secure XGB predict with the distributed model. Furthermore, by proposing secure permutation protocols, we can improve the training efficiency and make the framework scale to large dataset. We conduct extensive experiments on both public datasets and real-world datasets, and the results demonstrate that our proposed XGB models provide not only competitive accuracy but also practical performance.

==> HESS-XGB (2)/conclusion.tex <==
\section{Conclusion and Future Work}\label{conc}
In this paper, we propose an end-to-end framework for large-scale secure XGB under vertically partitioned data setting. 
With the help of secure multi-party computation technique, we first propose SS-XGB, a secure XGB training model.
We then propose HEP-XGB and CRP-XGB, which improves the efficiency of SS-XGB based on different realizations of secure permutation. 
We also propose a secure XGB prediction algorithm. 
The experimental results show that our proposed models achieve competitive accuracy with the plaintext XGB and can scale to large datasets.
%
In the future, we plan to further optimize the communication of the secret sharing protocols, which is the main bottleneck in our industrial test. %The framework can be repurposed for other machine learning applications and multi-party tasks.

%combining Homomorphic Encryption (HE) and Secret Sharing (SS), for two parties to build secure XGB   
%To do this, we first combined Homomorphic Encryption (HE) and Secret Sharing (SS), and proposed efficient computation primitives under these two domains and the transformation protocols. 
%Based on the hybrid-domain primitives, we implemented two secure XGB training algorithms, i.e., SS-XGB that uses SS only and HESS-XGB that employs both HE and SS, and one corresponding prediction algorithm.
%The complexity analysis shows that SS-XGB and HESS-XGB have their own advantages. We finally conducted experiments on benchmark dataset to verify the model performance and presented our real-world application. 
%In the future, we would like to focus on the parallel optimization for the proposed secure XGB algorithms and implement more secure machine learning algorithms for industrial applications based on the flexible framework.

==> HESS-XGB (2)/experiment.tex <==
\section{Experiments}\label{secexp}
% We demonstrate that HEP-XGB and CRP-XGB achieve a practical performance in terms of both accuracy and efficiency. We first present the accuracy evaluation and compare with primary XGB model. Then we vary the size parameters and network conditions to examine their effect on efficiency. Further we verify the resource consumed while training large-scale dataset. Finally, we display the result in our real-world scenario.
% \ccc{revise later}

In this section, we present the comprehensive experiments we conducted to study the effectiveness and efficiency of our proposed secure XGB algorithms.


\subsection{Experimental Setup}\label{secsetup}
\nosection{Implementation}
We use $k=128$ bits to represent the fixed-point secret sharing scheme, and 20 out of which are used for the fractional part. We use 64 bits to represent the plaintext data. Zero sharing technique is applied to reduce the interaction cost with the help of pseudo-random functions (PRF) \cite{mohassel2018aby3}. 
As for homomorphic encryption, we implement the Okamoto-Uchiyama scheme~\cite{okamoto1998new} based on \textit{libtomath}\footnote{https://github.com/libtom/libtommath} and the key size is set to 2,048 bit. 
%
HEP-XGB needs the transformation protocols and we have to deal with the security concern of random number generation. Following the analysis in \cite{pullonen2012design}, we pick the random number $r \in \mathbb{Z}_{2^{k+\sigma}}$. The probability of information leaking is then reduced to $2^{-\sigma}$, where we set $\sigma =40$.

\nosection{Environment}
We conduct experiments on the machines equipped with Intel(R) Xeon(R) Platinum 8,269CY CPU @ 2.50GHz$\times$32 and 128G of RAM. We simulate multiple parties by initializing multiple dockers with the given core limit. The network condition is manipulated with the traffic control command of Linux. To be specific, we consider the transmission $bandwidth$ and $latency$.

\nosection{Datasets}
We choose two types of datasets, which belong to different scales. 
First, we use four \textbf{public} benchmark datasets, including  Energy\footnote{https://www.kaggle.com/loveall/appliances-energy-prediction}  (regression task with 19,735 samples and 27 features), Blog\footnote{http://archive.ics.uci.edu/ml/datasets/BlogFeedback} (regression task with 60,021 samples and 280 features), Bank\footnote{http://archive.ics.uci.edu/ml/datasets/Bank+Marketing\#} (classification task with 40,787 samples and 48 features after preprocessing), and Credit\footnote{https://www.kaggle.com/uciml/default-of-credit-card-clients-dataset} (classification task with 30,000 samples and 23 features). The features are evenly divided into two parties. 
%
We split 80\% of the samples as training dataset, unless the division has been given. In terms of efficiency test, we generate synthetic data with \textit{sklearn}\footnote{https://scikit-learn.org/stable/} toolkit. 
%
Second, we use two \textbf{real-world} datasets, including a dataset for regression (617,248 samples for training and 264,536 samples for testing) and another dataset for classification (140,410 samples for training and 111,618 samples for testing). 
For the regression dataset, Party A holds 25 features and label, and Party B holds 29 features. For the classification dataset Party A holds 16 features and label, and Party B holds 7 features.

\nosection{Evaluation metrics}
For the four public datasets, we use Area Under the ROC Curve (AUC) as the evaluation metric for classification tasks, and use Root Mean Square Error (RMSE) as the metric for regression tasks.
For the two real-world datasets, besides AUC and RMSE, we also use four commonly used metrics in industry, including F1 score\footnote{https://en.wikipedia.org/wiki/F-score}, KS value\footnote{https://en.wikipedia.org/wiki/Kolmogorov\%E2\%80\%93Smirnov\_test}, coefficient of determination\footnote{https://en.wikipedia.org/wiki/Coefficient\_of\_determination} (R$^2$), and Mean Absolute Error (MAE). 
%
F1 and KS are used for classification task, while R$^2$ and MAE are used for regression task.

\subsection{Accuracy Comparison on Public Datasets}\label{secacc}

We compare accuracy with the plaintext XGB on the above four public datasets. During experiment, all the models share the same parameters. We set $max\_depth=5$ and the \textit{tree\_method} as `approx' in order to enable the quantile sketch splitting. We set the tree number as 30 and 20 for regression tasks and classification tasks, respectively. We repeat each experiment 6 times and report the average results in Table \ref{tab:acc}.

\begin{table}[t]
  \centering
  \caption{Accuracy comparison on public datasets.}
  \label{tab:acc}
%   \vspace{-0.15in}
    \begin{tabular}{lllll}
    \toprule
    \textbf{Dataset} & \textbf{XGB} & \textbf{SS-XGB} & \textbf{HEP-XGB} & \textbf{CRP-XGB} \\
    \midrule
    Energy   & 86.58608 & 87.44647 & 87.39388 & 87.39582 \\
    Blog  & 23.20011 & 23.12014  & 23.08946 & 23.05300 \\
    Bank  & 0.94543 & 0.94138 & 0.94125 & 0.94164 \\
    Credict & 0.78302 & 0.78344 & 0.78345 & 0.78344 \\
    \bottomrule
    \end{tabular}%
  \label{tab:accuracy}%
\end{table}%

In general, our three secure algorithms achieve competitive accuracy against the plaintext XGB model. We conclude that the slight loss is caused by two reasons. First, we adopt fixed-point representation, with narrower precision than plaintext float-point representation. Second, secure algorithms introduce function approximation (e.g., $sigmoid$) and probable failure of $truncation$ \cite{mohassel2017secureml}.

\subsection{Efficiency Analysis on Synthetic Dataset}\label{seceff}
We analyze model efficiency by conducting the following experiments. 
The basic settings are as follows: 
\begin{itemize}
    \item The dataset is generated with 5,000 samples and 250 features.
    \item We run 10 trees with depth as 4 and feature bucket is 10.
    \item Bandwidth is 100Mbps and latency is 5ms.
\end{itemize}
In each experiment, we vary one parameter and report the average time of the main steps in Algorithm \ref{alg:trainxgb}. Unless mentioned, the above basic settings are adopted.

\nosection{Effect of sample size, feature size, and bucket size}
We vary these size parameters and study their impacts on three secure XGB models. 
%
We report the time of $SumGradients$ for each model in Figure \ref{figexp_dataset}. %,, we report the time needed in the $SumGradients$ process, which is the divergence among the models. 
%
From it, we can see that (1) the running time of each model is proportional to the scale of data, i.e., sample size and feature size; 
%
(2) SS-XGB spends longer time with the increase of bucket number, the same as our analysis in Section \ref{secsp};
%
(3) in general, the optimized two variants, HEP-XGB and CRP-XGB, obtain similar efficiency and significantly outperform SS-XGB. 
%
Thus, we will mainly compare HEP-XGB and CRP-XGB in the following experiments.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{pics/exp_dataset.pdf}~
    \vskip -0.1in
    \caption{Effect of sample/feature/bucket size.}\label{figexp_dataset}
    % \vskip -0.05in
\end{figure}

\nosection{Effect of network parameters}
Because secret sharing plays a dominant role in our proposed models and it is a network sensitive scheme, we conduct detailed tests by varying the network parameters. 
%
To test \textit{bandwidth}, we set latency to 0 to get rid of its impact. 
%
Similarly, to test \textit{latency}, we use unlimited bandwidth.
%
We show the results in Figure \ref{figexp_net} and only report the most time-consuming steps for convenience. The $SumGradient$ implemented with HE based permutation is divided into three parts, i.e., $S2H$, $H2S$, and $HADD$. $S2H$ and $H2S$ are the transforming time cost between HE and SS, and $HADD$ denotes the time cost of accumulating the gradients under HE scheme, as described in Section \ref{secsp}.

From Figure \ref{figexp_net}, we can see that 
(1) \textit{CRP-SumG}, \textit{ComputeGain}, \textit{Argmax}, and $S2H$ are sensitive to bandwidth. %,, because they take more communications. 
% The bandwidth sensitive processes are \textit{CRP-SumG}, \textit{ComputeGain}, \textit{Argmax} and $S2H$, which takes more communications. 
%
Especially for \textit{CRP-SumG}, since it reveals mask permutation and mask share, which are proportional to the dataset size; 
In contrast, \textit{HEP-SumG} and its main subprocess \textit{HADD} are stable with the change of bandwidth. 
%
(2) with unlimited bandwidth, the time of each secret sharing process significantly decreases and CRP-based $SumGradient$ becomes more efficient than HEP-based one. 
\textit{CRP-SumG} performs the best when bandwidth is above 200 Mbps; 
%
(3) \textit{ComputeGain} and \textit{Argmax} are sensitive to latency, which indicates that one can optimize the round number in $Division$ and $Argmax$ to further improve efficiency.


%
% We can also find that, with unlimited bandwidth, the time of each secret sharing process significantly decreases and CRP-based $SumGradient$ becomes more efficient than HEP-based.
% %
% By varying latency, we can figure out the processes with many communication rounds, e.g. \textit{ComputeGain} and \textit{Argmax}. \ccc{cannot follow}
% %
% This suggests us to optimize the round numbers in $Division$ and $Argmax$ protocols.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{pics/exp_net.pdf}~
    \vskip -0.1in
    \caption{Effect of network ability.}\label{figexp_net}
    \vskip -0.05in
\end{figure}


\subsection{Comparison on Real-world Datasets}
We first show the accuracy comparison results in Table \ref{tab:realacc}, where the top one denotes the classification task and the bottom one denotes the regression task.  \textbf{XGB-PartyA} trains the plaintext XGB only with the features at Party A, while \textbf{XGB} uses the combined features of A and B. 
%
From Table \ref{tab:realacc}, we can see that 
(1) the joint models clearly improve the accuracy of XGB-PartyA, which proves the advantages of federated learning; 
%
(2) the accuracy of HEP-XGB and CRP-XGB is similar to XGB on the regression task but lower than XGB on the classification task.
%
We analyze the accuracy loss by replacing the secure $Sigmoid$ approximation with plaintext computation, and the AUC then goes up to 0.84463. 
%
This indicates that the approximation of $Sigmoid$ (described in Section \ref{secprot}) brings accuracy loss, especially when the dataset is large.

\begin{table}[t]
  \centering
  \caption{Accuracy comparison on real-world datasets.}
  \vspace{-0.15cm}
  \label{tab:realacc}
    \begin{tabular}{lllll}
    \toprule
    \textbf{Model} & \textbf{XGB-PartyA} & \textbf{XGB} & \textbf{HEP-XGB} & \textbf{CRP-XGB} \\
    \midrule
    \textbf{AUC} & 0.79904 & 0.84257 & 0.82945 & 0.83023 \\
    \textbf{KS} & 0.44735 & 0.52524 & 0.50270 & 0.50350 \\
    \textbf{F1 Score} & 0.20071 & 0.25190 & 0.24429 & 0.24504 \\
    \midrule
    \midrule
    \textbf{Model} & \textbf{XGB-PartyA} & \textbf{XGB} & \textbf{HEP-XGB} & \textbf{CRP-XGB} \\
    \midrule
    $R^{2}$ & 0.28634767 & 0.3324149 & 0.3312035 & 0.3320921 \\
    \textbf{RMSE} & 6459.2851 & 6246.4065 & 6253.0948 & 6248.9397 \\
    \textbf{MAE} & 2638.36573 & 2547.8378 & 2548.3600 & 2548.9299 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%

We then compare the efficiency of CRP-XGB and HEP-XGB on the classification dataset under three typical environment settings:
\begin{itemize}
    \item \textbf{S1}: 32 cores, bandwidth 10 Gbps + latency 0.1 ms; %\Simley{0.5}
    \item \textbf{S2}: 32 cores, bandwidth 100 Mbps + latency 5 ms; %\Simley{0}
    \item \textbf{S3}: 8 cores, bandwidth 20 Mbps + latency 50 ms. %\Simley{-0.5}
\end{itemize}

We report the average training time per tree for HEP-XGB and CRP-XGB in Table \ref{tab:timetest}. 
%
From it, we can see that 
(1) the training time of CRP-XGB and HEP-XGB increases rapidly under bad network condition (\textbf{S3}), which indicates that both CRP-XGB and HEP-XGB rely much on the network ability; 
%And the computation intensive process ($HADD$) is not the bottle neck even with bad parallelism (S3). 
(2) CRP-XGB is a better choice under good network conditions. For example, CRP-XGB is about 10 times faster than HEP-XGB under \textbf{S1}; 
(3) HEP-XGB outperforms CRP-XGB under bad network conditions, e.g., HEP-XGB saves the running time by 26.5\% under \textbf{S3}.

\begin{table}[t]
  \centering
  \caption{Time test on real-world dataset}
  \label{tab:timetest}
    \begin{tabular}{llll}
    \toprule
    \textbf{Model} & \textbf{S1} & \textbf{S2} & \textbf{S3} \\
    \midrule
    \textbf{CRP-XGB} & 5.1s   & 155.8s & 857.4s \\
    \textbf{HEP-XGB} & 47.6s  & 151.0s & 630.8s \\
    \bottomrule
    \end{tabular}%
\end{table}%

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{pics/exp_pct.pdf}~
%     \vskip -0.1in
%     \caption{Time Test on Real-world Dataset}\label{figexp_pct}
%     \vskip -0.05in
% \end{figure}


\subsection{Scalability Test}
To test the scalability of CRP-XGB and HEP-XGB, we compare their resource consumption based on the experimental environment reported in Section \ref{secsetup}. 
%
% is another critical factor for large-scale training, so we conduct experiments to compare the scalability of CRP-XGB and HEP-XGB in the LAN setting. 
%
To do this, we generate a dataset with 12,000,000 samples and 200 features (considering the memory limit). We train two trees for each model and record their resource usage in Figure \ref{figexp_res}, where we use local area network. 
%
From it, we can see that (1) both CRP-XGB and HEP-XGB can scale to tens of millions of datasets; 
(2) in general, CRP-XGB uses much less CPU than HEP-XGB, because HEP-XGB involves time-consuming HE operations. 
%
The results indicate that, compared with HEP-XGB, CRP-XGB is more suitable for the situations where the network ability is good. 

% CRP-XGB is computation friendly and only uses (about 60\%) less memory.
%The CPU usage peaks of CRP-XGB are caused by the serialization and deserialization. HEP-XGB have heavy homomorphic encryption computations.  In terms of memory, because the ciphertext is much longer than secret shares, 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{pics/exp_resource.pdf}
    \vskip -0.1in
    \caption{Resource consumption. Left Figure: CRP-XGB, right figure: HEP-XGB.}\label{figexp_res}
    \vskip -0.05in
\end{figure}

% In this section, we first analyze the choice for Homomorphic Encryption.
% Then we study the performance and usability of our secure XGB on a benchmark dataset. 
% Finally, we present how is secure XGB applied in our real-world scenario.

% \subsection{Choice of Homomorphic Encryption}
% Homomorphic Encryption plays a key role in the HESS-XGB, so it is critical to the choose and configure the algorithm. As the previous description in section \ref{secimp}, we implement two of the most popular algorithms, Paillier and OU, based on libtommath\footnote{https://github.com/libtom/libtommath}. 

% We first compare their running time of \textbf{Enc}ryption, \textbf{Dec}ryption and \textbf{H}omomorphic \textbf{Add}ition, which are dominated by the key size ($l \in \left\{1024, 2048, 3072\right\}$). We repeat each of the operations for 100,000 times and report the total time (in seconds) in Table \ref{tab:hetime}, where factor denotes the speedup of OU against Paillier. We find that OU outperforms Pailler over all the operations, and therefore we choose OU in practice.  
% %abundant computations in machine learning algorithms. 
% We also note that the running time grows rapidly with the increase of key size. In practice, $l=2048$ turns out to be a good choice that meets the requirements for both security and efficiency.

% \begin{table}[htbp]
%   \centering
%   \caption{Time Test for HE (in seconds)}
%   \vspace{-0.15in}
%     \begin{tabular}{lllll}
%     \toprule
%     \textbf{HE Setting} & \textbf{Enc} & \textbf{HAdd1}$^\star$ & \textbf{HAdd2}$^\dagger$ & \textbf{Dec} \\
%     \midrule
%     OU-1024 & 86.285 & 0.311 & 2.388 & 9.889 \\
%     Paillier-1024 & 306.104 & 1.003 & 311.189 & 300.560 \\
%     Factor & 3.55x & 3.22x & 130.31x & 30.39x \\
%     \midrule
%     OU-2048 & 432.241 & 0.914 & 8.785 & 28.773 \\
%     Paillier-2048 & 1739.590 & 2.227 & 1754.110 & 1966.790 \\
%     Factor & 4.02x & 2.44x & 199.68x & 68.35x \\
%     \midrule
%     OU-3072 & 2147.340 & 1.946 & 19.680 & 62.241 \\
%     Paillier-3072 & 8344.960 & 6.549 & 8404.650 & 8759.290 \\
%     Factor & 3.89x & 3.36x & 427.06x & 140.73x \\
%     \bottomrule
%     \end{tabular} \\
%     \footnotesize{$^\star$ \textit{ciphertext+ciphertext} \quad $^\dagger$\textit{ciphertext+plaintext}} \\
%   \label{tab:hetime}%
% \end{table}%
% \vspace{-0.1in}

% \subsection{End-to-end Accuracy Comparison}
% \label{secauc}

% \nosection{Settings}
% To compare our secure XGB with the plaintext XGB in terms of performance, 
% %In order to put the secure XGB algorithm into industrial use, 
% we conduct a contrast experiment on the Mnist dataset\footnote{http://yann.lecun.com/exdb/mnist/}, which is widely used in privacy-preserving machine learning testing \cite{mohassel2017secureml}. 
% The Mnist dataset has 60,000 training samples and 10,000 testing samples and each sample is a image of a handwritten digit from 0 to 9. The grayscale levels of $28\times 28$ pixels make up the 784 features, which are vertically split into two parties evenly, i.e., we assume each party has 392 features. We take the digits from 0-4 as positive samples and others as negative ones. Then it becomes a standard binary classification task. We use Area Under the ROC Curve (AUC) as the evaluation metric. 
% During comparison, we set the same parameters for all the algorithms. We set learning rate to 0.3 and sampling rate to 0.7 (for both samples and features). 

% % and compare the key performance measurement (AUC) for classification problems. We experiment on the Mnist dataset\footnote{http://yann.lecun.com/exdb/mnist/}, which is widely used in machine learning testing. There are 60,000 training samples and 10,000 testing samples and each sample is a image of a handwritten digit from 0 to 9. The grayscale levels for $28\times 28$ pixels make up the 784 features, which are vertically split into two computation parties. And we transform the digits that are above number 4 to be positive samples or negative samples otherwise. Then it becomes a standard binary classification task. The algorithms share some predetermined parameter settings. We set learning rate as 0.3 and sampling rate as 0.7(for both samples and features).

% \nosection{Results and analysis}
% We summarize the comparison results in Table \ref{tab:auc}. Note that both SS-XGB and HESS-XGB achieves the same accuracy.  We can see that our proposed secure XGB converges slower than original XGB, and eventually the AUC of secure XGB is comparable but a little bit lower than that of XGB (0.973539 vs. 0.978956). This is because secure XGB has some nonlinear computation primitives (e.g. division \& sigmoid) which have to be computed approximated. 
% % Due to the function approximated securely. ion primitives (e.g. division \& sigmoid)% and lack of pruning
% % , the secure XGB converges slower than original XGB.  But our secure XGB algorithms finally approach to the results of original XGB. 
% The little performance loss is totally acceptable, especially considering its privacy preserving ability. % with the data privacy in return.

% \begin{table}[t]
%   \centering
%   \caption{AUC test for Secure XGB}
%   \vskip -0.1in
%     \begin{tabular}{lccc}
%     \toprule
%     \textbf{Secure XGB} & dep=3 & dep=4 & dep=5 \\
%     \midrule
%     n\_tree=5 & 0.848859 & 0.871682 & 0.908069 \\
%     n\_tree=10 & 0.870559 & 0.910726 & 0.937391 \\
%     n\_tree=20 & 0.899864 & 0.938292 & 0.963428 \\
%     n\_tree=30 & 0.920106 & 0.952357 & 0.973539 \\
%     \midrule
%     \midrule
%     \textbf{XGB} & dep=3 & dep=4 & dep=5 \\
%     \midrule
%     n\_tree=5 & 0.855560 & 0.897462 & 0.931451 \\
%     n\_tree=10 & 0.892414 & 0.929320 & 0.958429 \\
%     n\_tree=20 & 0.917860 & 0.954457 & 0.971062 \\
%     n\_tree=30 & 0.934475 & 0.967075 & 0.978956 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:auc}%
% \end{table}%

% \subsection{Efficiency Comparison}
% %\vskip -0.15in
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.43\textwidth]{pics/band.pdf}~
%     \vskip -0.1in
%     \caption{Bandwidth Test for HESS and SS }\label{figband}
%     \vskip -0.05in
% \end{figure}

% Efficiency is another important factor for practical use. We compare the running time of the proposed
% two method: SS-XGB and HESS-XGB. The comparison is carried out on a fraction of the Mnist dataset (with 1,000 samples).
% We apply the two algorithms by varying bandwidth in $\left\{10, 20, 30, 40, 60, 80, 100\right\}$ and set
% the network delay to 5ms. The algorithm parameters are the same as section \ref{secauc}
% except that the tree depth is fixed to 4. 
% We report the average training time for a single tree in Figure \ref{figband}.
% From it, we conclude that HESS-XGB works better than SS-XGB on Mnist dataset, especially with the decreasing of bandwidth. 
% %It works better for machine learning tasks and runs $2\sim3\times$ faster in our real applications. 
% The result arrives the same conclusion as our complexity analysis in section \ref{seccomp}. For a specific task, in practice, one can substitute the data
% size \& operation time in Table \ref{tab:hetime} to choose the appropriate algorithm (i.e., SS-XGB or HESS-XGB). 


% Moreover, we observe that HESS-XGB is more memory friendly. Take Mnist dataset for example, the peak memory of HESS-XGB is only half of SS-XGB. 
% This is because HESS-XGB stores the local features in sparse matrices by taking advantage of the vertical data partition setting. 
% This is a delightful character, considering XGB algorithm cannot train in a mini-batch way. With a lower memory cost, HESS-XGB is able to supports larger datasets. 

% Finally, in order to better study the efficiency of HESS-XGB and clarify future improvements,
% we analyze its time allocated during training procedure. 
% From Figure \ref{figoptime}, we find that around 80\% of the time spends on cumulating the encrypted values (\textbf{HADD}, line 16-17) in Algorithm \ref{alg:hessbuck}, and over 10\% of the time is on encrypting $g \& h$ (\textbf{A2H}, line 5-8) in Algorithm \ref{alg:hessbuck}. 
% %It takes most of the time to encrypt the g \& h(line 5-8) and cumulate the encrypted values(line 16-17) in Algorithm \ref{alg:hessbuck}. 
% The above results shed light on how to further improve the efficiency of HESS-XGB for industrial practitioners, i.e., parallelize encryption and
%  node splitting.
% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=0.4\textwidth]{pics/optime.pdf}
% 	\vskip -0.15in
% 	\caption{Operation time percentage during training}\label{figoptime}
% 	\vskip -0.1in
% \end{figure}

% \subsection{Application}
% We deploy our proposed secure XGB into real-world fraud detection task for online payment services. As a payment platform, we facilitate online transaction service and obtain
% the historical information for the customers. 
% Traditionally, we build our own risk control model using XGB. However, the merchants also have private transaction data that could be used to further improve 
% risk control ability. 
% But the data is not allowed to share for the sake of user privacy and commercial principles. 
% With secure XGB, we can build secure risk control model together with the merchants. 
% Our data for this task contains 100,000 samples (70\% as training data) and 50 selected features. The AUC of our individual XGB model is 0.9778. With extra 30 features from the merchant, the AUC of secure XGB is improved to 0.9924. The joint model can detect more potential frauds and significantly reduce capital loss.



==> HESS-XGB (2)/intro.tex <==
\section{Introduction}\label{intro}
With the concern of data privacy and the requirement of better machine learning performance, %which are collaboratively built by multiple parties, 
Privacy Preserving Machine Learning (PPML) \cite{mohassel2017secureml}, which enables multiple parties jointly build machine learning models privately, has been drawing much attention recently. To date, most existing PPML models only focus on linear regression \cite{hall2011secure,gascon2017privacy}, logistic regression \cite{mohassel2017secureml,kim2018secure}, and neural network \cite{wagh2018securenn,rachuri2019trident,zheng2020industrial}. 
They are mainly divided into two types based on how data is partitioned, i.e., horizontally partitioned PPML that assumes each party has a subset of the samples with the same features, and vertically partitioned PPML that assumes each party has the same samples but different features \cite{yang2019federated}. The former usually appears when participants are individual customers (2C), while the latter is more common when participants are business organizations (2B). In this paper, we focus on the later setting. 

Gradient tree boosting is one of the widely used type of machine learning models that shine in different fields, e.g., fraud detection \cite{rushin2017horse}, recommender system \cite{zhang2018industrial}, and online advertisement \cite{ling2017model}. 
As an optimized implementation, XGB \cite{chen2016xgboost} achieves promising results in various competitions and real-world applications, since it is a gradient boosting model whose key idea is applying numerical optimization in function space and optimizing over the cost functions directly \cite{friedman2001greedy}. 
Therefore, how to build privacy preserving XGB with vertically partitioned data is an important research topic. 

So far, there are several existing researches on privacy preserving gradient tree boosting \cite{liu2019boosting,li2019practical,fengy2019securegbm,cheng2019secureboost}. Among them, \cite{liu2019boosting,li2019practical} are built for horizontally partitioned data setting. Although privacy preserving XGB are proposed for vertically partitioned data setting in \cite{fengy2019securegbm,cheng2019secureboost}, they are not provable secure. Specifically, intermediate information, e.g., the sum of the first and second order gradients for each split and the order of split gains, is revealed during model training procedure.

Building a secure XGB is challenging due to the following reasons. 
(1) \textit{Complicated computation primitives}. Unlike other machine learning models such as logistic regression which only require secure matrix \texttt{addition} and \texttt{multiplication} primitives, XGB needs additional non-linear computation primitives, e.g., \texttt{division} and \texttt{argmax}. 
(2) \textit{High memory cost}. Most models such as neural network are suitable for mini-batch training, that is, only a small batch of samples are loaded in each training iteration, and thus they do not need large memory to support large-scale datasets. In contrast, XGB uses (sampled) full-batch dataset to build trees. Therefore, how to save memory cost is the key to large-scale secure XGB.

To solve the above challenges, in this paper, we propose to build large-scale secure XGB by leveraging hybrid secure multi-party computation techniques. 
Our key idea is taking XGB as a function that two vertically partitioned parties want to compute securely, during which %only input and the output are revealed to each party and 
all the information is either secretly shared or encrypted, except for the trained model as the function output. 
To be specific, we first propose a secure XGB training approach, which relies on secret sharing scheme only and serves as a baseline, and we call it as SS-XGB. 
%
SS-XGB is provable secure but cannot scale to large datasets since it introduces redundant computations for security concern. %
We then improve the efficiency of SS-XGB by leveraging secure permutation protocol. 
%
We also propose two realizations of secure permutation, based on Homomorphic Encryption (HE) and Correlated Randomness (CR), and term the secure XGBs with these two secure permutation protocols as HEP-XGB and CRP-XGB, respectively. 
%
HEP-XGB is computational intensive which makes it a good choice under bad network condition. CRP-XGB, in contrast, needs less computation resources (e.g., CPU and memory) and enjoys an attractive performance with high bandwidth.  
% \ccc{HEP-XGB can ...}
%
% \ccc{SSP-XGB can ...}
%
% present two security domains, i.e.,  Homomorphic Encryption (HE) and Secret Sharing (SS). Both domains provide efficient computation primitives, e.g., \texttt{HADD} and \texttt{SADD} which are the addition primitives under HE domain and SS domain respectively. Then, we propose transformation primitives between these two domains, i.e., \texttt{H2S} and \texttt{S2H}. 
% We set up a secure framework with both security domains and implement two secure XGB training algorithms with the primitives, i.e., SS-XGB within SS domain only and HESS-XGB that employs both HE and SS domains. SS-XGB is computationally efficient but sustains high communication cost when handling sparse features, which is usually the bottleneck of PPML in practice. In contrast, HESS-XGB cuts down the communication cost by involving extra encryption/decryption operations. 
After training, each party holds a partial tree structure and secretly shared leaf weights. 
Next, we present a secure XGB prediction algorithm for two parties to jointly make predictions with their local features, tree structures, and leaf weights. 
% We also present how to implement SS-XGB \& HESS-XGB and analyze their complexities. 
Finally, we verify our model performance by conducting experiments on public and real-world datasets and explaining our real-world applications. 
%
We summarize our main contributions below:
\begin{itemize} [leftmargin=*] \setlength{\itemsep}{-\itemsep}
% \item We propose to combine the two classical security computation domains (i.e., HE and SS) so as to deal with secure machine learning tasks. Our hybrid-domain framework can significantly boost the efficiency of sparse matrix multiplication, which makes it practical for industrial scenarios. 

\item We propose an end-to-end secure XGB framework by leveraging hybrid secure multi-party computation techniques, which includes model training, model storage, and model prediction. 

% \item We design novel secure XGB training algorithms (SS-XGB and HESS-XGB) and corresponding prediction algorithm based on the framework.To the best of our knowledge, it is the first provable secure XGB under semi-honest adversaries in literature. We also analyze the complexity of SS-XGB and HESS-XGB, which is a selection guide given the dataset and specified environment settings (e.g., %memory and network status).  

\item We propose two secure permutation protocols to further improve the efficiency of SS-XGB. 

\item We conduct experiments on public and real-world datasets, and the results demonstrate the effectiveness and efficiency of our proposed secure XGB algorithms. %Our real-world application also shows the feasibility of our proposal.

% \item We propose a hybrid secure multi-party computation protocol by combining HE and SS, which supports flexible computation primitives and their 
% transformations. The hybrid protocol can be employed to build any machine learning models. 
% \item We propose novel secure XGB training algorithms (SS-XGB and HESS-XGB) and prediction algorithm based on the hybrid protocol. Our complexity analysis indicates that SS-XGB has better performance when datasets are small and network status is good, while HESS-XGB is more suitable for large-scale datasets and poor network status due to its low memory cost and small communication cost. To the best of our knowledge, we are the first provable secure XGB under semi-honest adversaries in literature. 
% \item We conduct extensive experiments on real-world datasets and the results demonstrate the effectiveness and efficiency of our proposed secure XGB.
\end{itemize}

==> HESS-XGB (2)/preliminary.tex <==
\section{Preliminary}\label{secpre}
% In this section, we first declare the algorithm target and corresponding data setting. The computations are executed interactively by data providers with the help of an aided server. Then, we define the output model as well as the security setting. Finally, the key derivation of XGB algorithm is analyzed for further descriptions. 

%, which is necessary for the following pseudocodes.
% Further, the computation primitives in use are described in the final part and related simplified
% notations are applied in the pseudocodes. With the notations, we can get rid of the distributed
% computation details and provide a high-level description for the algorithm.

%In this section, we describe the problem setting, background knowledge on XGB, security domains, and computation primitives.

\subsection{Settings}

\nosection{Scenario setting}
Our proposal is designed for two parties (A \& B), who partition data \textit{vertically}, to jointly build secure XGB model. 
%
That is, A and B have aligned their common samples but they have different features. 
% Our proposal utilizes the data from two parties (A \& B) to build a XGB model securely.
%The model is partially held by both parties and applied to predict on the new samples.
%We focus on two-party computation and will generalize to multi-party in later discussion.
% Two joint parties A \& B align their common samples and obtain different features.
% In this way, the dataset is regarded as \textit{vertically partitioned}. 
Formally, let $X^{M\times N}$ be the original feature matrix with $M$ and $N$ denoting the number of samples and features, respectively. 
Under vertical FL setting, $X^{M\times N}$ is distributed to A and B, A has a feature matrix $X_{A}^{M\times N_{A}}$, and B has the other feature matrix $X_{B}^{M\times N_{B}}$, where $N_{A}$ and $N_{B}$ denote the number of features at Party A and Party B, such that $N=N_{A}+N_{B}$. 
% The feature matrix $X_{M\times N}$, with $M$ samples, is represented by two 
% matrices $(X_{A})_{M\times N_{A}}$ and $(X_{B})_{M\times N_{B}}$, 
% where $N=N_{A}+N_{B}$ is the total feature number. 
%
We also assume one of the parties (e.g., Party A) holds the label vector $Y$. 

\nosection{System setting}
Besides the above two parties (A and B), we also employ a trusted dealer (C) to generate correlated randomness, e.g., Beaver triplet \cite{beaver1991efficient}, following the \textit{MPC with pre-processing} paradigm \cite{ishai2013power,mohassel2017secureml}. 
%
We introduce a secure hardware (i.e., Intel SGX) to play the role of C, in order to enable more efficient and scalable MPC. 
%This is a 3-party framework, similar to ABY \cite{mohassel2018aby3}, except that 
C is only responsible for randomness generation and has no access to the inputs and outputs of A and B.
The input-independent randomness can be massively produced by C before training starts and will be consumed by A and B during the training process. 
%The aim of this aided server is simplifying the computation of the input parties. 
% We will show the details in Section \ref{secxgb}.
% A matrix or vector is denoted by braces and subscripted 
% by the data size. While referring to a specific element, we write a representative element
% in lowercase and a superscript with its indexes, e.g. $ X_{A} :\{x_{A}\}^{i,j}$. 

\nosection{Model setting}
For security, we distribute the model to two parties after training. 
%
Both parties share the same tree structures, but none of them has the whole split information. 
%
Specifically, the split information on a single node will only be visible to the party who owns the corresponding feature, and will be non-visible (dummy node) to the other party. 
%
Moreover, both parties collaboratively store the leaf weights in secret sharing scheme. 
%
To this end, we can avoid potential information leakage from the trained model.

\nosection{Security setting}
Our proposal enjoys information-theoretic security and is secure in the semi-honest adversarial setting. That is, the adversary is not restricted to be a probabilistic polynomial time algorithm, and tries to infer information although it strictly obeys the execution protocol. 
This setting is adopted by most existing secure machine learning models \cite{mohassel2018aby3,mohassel2017secureml,wagh2018securenn}.
%\ccc{may need to explain the third-party server}

\subsection{XGB}
XGB follows the gradient boosting framework and applies numerical optimization in function space~\cite{friedman2001greedy}. 
In machine learning, the learning task is based on the definition of the loss function.
The loss function $l(y, \hat{y})$ is defined to measure the difference between the label $y$ and the estimation $\hat{y}$.

As an addictive model, XGB~\cite{chen2016xgboost} minimizes the loss sum of all the samples 
as objective iteratively.
For each tree fitting, the algorithm first calculates necessary statistics, i.e., the first-order gradient $g_i$ and second-order gradient $h_i$ of sample $i$:
\begin{equation}
g_i=\partial_{\hat{y}_i^{(t-1)}} l(y_i, \hat{y}_i^{(t-1)}), \quad h_i=\partial_{\hat{y}_i^{(t-1)}}^2 l(y_i, \hat{y}_i^{(t-1)}),
\end{equation}
where $\hat{y}_i^{(t-1)}$ is the prediction by the end of last iteration.

Then the gradient sums can be cumulated for the instance set $I_j$ on each node j:
 \begin{equation}
G_j = \sum_{i\in I_j} g_i, \quad H_j = \sum_{i\in I_j} h_i.
\end{equation}
%Where $g_i$ and $h_i$ are the first-order and second-order gradients of sample $i$ in the j-th node $I_j$.

% The objective for the t-th iteration is then represented as:
% \begin{equation}
% \begin{split}
% \text{obj}^{(t)} & = \sum_{i=1}^M l(y_i, \hat{y}_i^{(t)}) + \sum_{i=1}^t\Omega(f_i) \\
%           & = \sum_{i=1}^M l(y_i, \hat{y}_i^{(t-1)} + f_t(x_i)) + \Omega(f_t) + \mathrm{constant}
% \end{split}
% \end{equation}
% Then it takes the second-order Taylor expansion approximation of loss 
 %and removes the constant term:
%  \begin{equation}
%   \begin{split}
%  \text{obj}^{(t)} &=\sum_{i=1}^M [l(y_i, \hat{y}_i^{(t-1)}) + g_i f_t(x_i) + \frac{1}{2} h_i f_t^2(x_i)] + \Omega(f_t) + \mathrm{constant}\\
%  			&\approx\sum_{i=1}^M [g_i f_t(x_i) + \frac{1}{2} h_i f_t^2(x_i)] + \Omega(f_t)
%   \end{split}
%  \end{equation}
 It takes the second-order Taylor expansion approximation of objective and adds regularization to the model.
The optimal leaf weight $w_j^\ast$ and objective $\text{obj}^\ast$ are solved with regard to the objective function:
\begin{equation}
\label{eqweight}
w_j^\ast = -\frac{G_j}{H_j+\lambda},
\end{equation}
\begin{equation}
\label{eqobj}
\text{obj}^\ast = -\frac{1}{2} \sum_{j=1}^T \frac{G_j^2}{H_j+\lambda} + \gamma T,
\end{equation}
where $\gamma$ and $\lambda$ are the regularizers for the leaf number and leaf weights respectively.
Equation (\ref{eqobj}) is applied to measure a split proposal at each node and determines the tree structure. 
With Equation (\ref{eqweight}), the leaf weights are finally acquired.
%  \begin{equation}
%   g_i = \partial_{\hat{y}_i^{(t-1)}} l(y_i, \hat{y}_i^{(t-1)}), \quad h_i = \partial_{\hat{y}_i^{(t-1)}}^2 l(y_i, \hat{y}_i^{(t-1)})
% \end{equation}

% When the base learner $f_{t}$ is regression tree,  the prediction score is the corresponding leaf weight $w_{q(x)}$.
% Function $q$ directs a data point $x$ to a leaf node.  
% $\varOmega$  regularizes the number of leaf nodes $J$ and leaf weights $w_j$:
%  \begin{equation}\label{eq:xgb:obj}
%  \text{obj}^{(t)} \approx \sum_{i=1}^M [g_i w_{q(x_i)} + \frac{1}{2} h_i w_{q(x_i)}^2] + \gamma J + \frac{1}{2}\lambda \sum_{j=1}^J w_j^2
% \end{equation}
% Where $ \gamma$ and $\lambda$ are the regularizer weights.

% Further, the objective terms can be regrouped by the leaves:
% \begin{equation}
% \begin{split}
%  \text{obj}^{(t)} &\approx\sum^J_{j=1} [(\sum_{i\in I_j} g_i) w_j + \frac{1}{2} (\sum_{i\in I_j} h_i + \lambda) w_j^2 ] + \gamma J \\
%  &= \sum^J_{j=1} [G_jw_j + \frac{1}{2} (H_j+\lambda) w_j^2] +\gamma J
%  \end{split}
% \end{equation}
% Where $G_j$ and $H_j$ sum the statistics of sample set of the j-th leaf $I_j$:
% \begin{equation}
% G_j = \sum_{i\in I_j} g_i, \quad H_j = \sum_{i\in I_j} h_i
% \end{equation}

% With regard to this quadratic form of independent $w_j$, the best leaf weight and objective are solved:
% \begin{equation}
% \label{eqweight}
% w_j^\ast = -\frac{G_j}{H_j+\lambda}
% \end{equation}
% \begin{equation}
% \label{eqobj}
% \text{obj}^\ast = -\frac{1}{2} \sum_{j=1}^T \frac{G_j^2}{H_j+\lambda} + \gamma T
% \end{equation}



% \subsection{Security Domains}
% Our proposed framework combines \textit{Homomorphic Encryption} and \textit{Secret Sharing},
% which are used as standalone solutions to security multi-party computation. Both methods provide secure computation environments for variables, so we introduce the concept \textit{Security Domain}
% to distinguish variables in different environments.
% There are three variable types and the security requirements:
% %\begin{itemize}
% 	%\item 
	
% 	\textbf{\textit{Norm}}: the \textit{Normal} variable $x$ can be a private variable of 
% 	one party or a public constant shared by both parties, e.g., the original private feature matrix held by party A or the public learning rate of the algorithm. 
% 	These variables can only be revealed to the party who owns them, but not to the other party.
% 	%\item 
	
%     \textbf{\textit{HE}}: the variables protected by \textit{Homomorphic Encryption} schema.
% 	Both parties exchange their Public Key $PK_{A}$ \& $PK_{B}$ with each other. 
% 	We denote variables under HE domain by square brackets, e.g. $[x]_{A}$, which stands for the ciphertext of $x$
% 	encrypted by $PK_{A}$ and can be decrypted by Secret Key $SK_{A}$.
% 	%This environment protects the \textit{Normal} variable $x$.%, which could be a private variable or an intermediate value.
% 	There are two requirements to ensure the domain security. Firstly, if the original data holder and the encrypter are not
% 	the same party, the cipertext cannot be accessed by the encrypter. Secondly, the encrypted intermediate values
% 	computed by the original variables by different parties cannot be access by the encrypter. The typical computation schema
% 	in this domain is regarding one party as an encrypter and the other as a calculator. All the computations is conducted by the calculator with ciphertexts. Because the calculator party has no access to the secret key of encrypter party,
% 	the original variables and computations are secure.
% 	%\item 
	
% 	\textbf{\textit{SS}}: the variable in \textit{Secret Sharing} domain is denoted
% 	by angle brackets, e.g. $\langle x\rangle$, which consists of two random shares $\langle x\rangle_{A}$
% 	and $\langle x\rangle_{B}$ physically distributed at the two parties. According to the definition of additive secret sharing,
% 	we have $x = \langle x\rangle_{A}+\langle x\rangle_{B}~mod~2^k$ to reconstruct the original variable, where $2^k$ is the size of finite field. Note that we omit $2^k$ for conciseness below.  
% 	%There are a series of protocols that conduct secure computations with SS variables by exchanging messages and some local computations.
% 	In SS domain, the messages are random values and reveal nothing about original data.
% 	To maintain the security of private variables, the share of the original data holder cannot be get by the other party. Besides, the shares of the intermediate values on both parties cannot be exchanged.
% %\end{itemize}

% In order to make use of the characteristics of both domains, variables are transformed between two domains when specific optimization is needed.
% \subsection{Computation Primitives}\label{secprimitive}
% %In the algorithm design, the secure computations are based on the protocols in single security domain.

% %Because the computation protocols are classical MPC primitives,only the primitive functionalities are listed here and the protocol details are neglected. 
% We introduce the brokenbar to separate the data hold by two parties, i.e., $(party\ A \text{\ \textbrokenbar\ } party\ B)$. 
% %the inputs and outputs to express the data distribution, $(party\ A \text{\ \textbrokenbar\ } party\ B)$. 
% For example, $(\left\langle x\right\rangle_{A} \text{\ \textbrokenbar\ } \left\langle x\right\rangle_{B}, [y]_{A})$ 
% means party A obtains the one partial share of $x$ and party B obtains the other partial share of $x$
% along with the cipertext of $y$ encrypted by $PK_{A}$. 
% We then present the computation primitives used in this paper as follows. 
% %There are several computation primitives are necessary for XGB:

% %\begin{itemize}
% 	%\item 
	
% 	\textbf{N2S}: Transforms a \textit{Norm} variable $x$ into a \textit{SS} variable with two shares($\left\langle x\right\rangle _{A}$ \& $\left\langle x\right\rangle _{B}$), having $  x = \left\langle x\right\rangle _{A}+ \left\langle x\right\rangle _{B}$:
% 	\begin{equation}
% 	\textit{N2S}: x\mapsto\left( \left\langle x\right\rangle _{A}\text{\ \textbrokenbar\ } \left\langle x\right\rangle _{B}\right),
% 	\end{equation}
% 	where one share is randomly generated in the finite field and the other is computed by subtraction.
% 	The variables are privately held by two parties 
% 	as a \textit{SS} variable for further secure computations. %The protocol inits a random value at the data holder as its partial share. Then it subtracts the value from origial variable and send the result to the other party as another random share. 
% 	We denote the transformation as $\left\langle x\right\rangle=N2S(x)$ for simplicity.
	
% 	%\item 
	
% 	\textbf{HADD}: Add two \textit{HE} variables and get the ciphertext of their original sum as the result, having $z=x+y$:
% 	\begin{equation}
% 	\begin{split}
% 	\textit{HADD}: (\text{\ \textbrokenbar\ } [x]_{A}, [y]_{A})\mapsto(\text{\ \textbrokenbar\ } [z]_{A} ), \\
% 	\textit{HADD}: ( [x]_{B}, [y]_{B}\text{\ \textbrokenbar\ })\mapsto( [z]_{B} \text{\ \textbrokenbar\ }).
% 	\end{split}
% 	\end{equation}
% 	Here, one party acts as the encrypter, and the other party adds the ciphertexts using additive homomorphic encryption. 
% 	%This operator chooses one party as encrypter and adds the ciphertext utilizing additive homomorphic encryption on the other party, i.e. the calculator party. 
% 	We denote the computation as $[z]_{A}=[x]_{A}+[y]_{A}$ for simplicity.
	
% 	%\item 
	
% 	\textbf{SADD}: Add two \textit{SS} variables and get a new \textit{SS} variable of their original sum as the result, having $z=x+y$:
% 	\begin{equation}
% 	\textit{SADD}: (\left\langle x\right\rangle_{A}, \left\langle y\right\rangle_{A} \text{\ \textbrokenbar\ }
% 	\left\langle x\right\rangle_{B}, \left\langle y\right\rangle_{B}
% 	)\mapsto( \left\langle z\right\rangle_{A} 
% 	\text{\ \textbrokenbar\ }
% 	 \left\langle z\right\rangle_{B} ) .
% 	\end{equation}
% 	This can be done by summing the local partial shares of the two inputs, i.e. $\left\langle z\right\rangle_{A} = \left\langle x\right\rangle_{A} +\left\langle y\right\rangle_{A}, \left\langle z\right\rangle_{B} = \left\langle x\right\rangle_{B} +\left\langle y\right\rangle_{B}$. 
% 	%$\left\langle z\right\rangle_{A}$ and $\left\langle z\right\rangle_{B}$ forms a legel pair of random shares for the result $z$.
% 	We denote the computation as $\left\langle z\right\rangle=\left\langle x\right\rangle+\left\langle y\right\rangle$ for simplicity.
	
% 	%\item 
	
% 	\textbf{SSUB}: Compute the subtraction for two \textit{SS} variables and get a new \textit{SS} variable of their original difference as the result, having $z=x-y$:
% 	\begin{equation}
% 	\textit{SSUB}: (\left\langle x\right\rangle_{A}, \left\langle y\right\rangle_{A} \text{\ \textbrokenbar\ }
% 	\left\langle x\right\rangle_{B}, \left\langle y\right\rangle_{B}
% 	)\mapsto( \left\langle z\right\rangle_{A} 
% 	\text{\ \textbrokenbar\ }
% 	\left\langle z\right\rangle_{B} ). 
% 	\end{equation}
% 	Similarly to \textit{SADD}, we denote the computation as $\left\langle z\right\rangle=\left\langle x\right\rangle-\left\langle y\right\rangle$ for simplicity.
	
% 	%\item 
	
% 	\textbf{SMUL}: Multiply two \textit{SS} variables and get a new \textit{SS} variable of their original product as the result, having $z=x\cdot y$:
% 	\begin{equation}
% 	\textit{SMUL}: (\left\langle x\right\rangle_{A}, \left\langle y\right\rangle_{A} \text{\ \textbrokenbar\ }
% 	\left\langle x\right\rangle_{B}, \left\langle y\right\rangle_{B}
% 	)\mapsto( \left\langle z\right\rangle_{A} 
% 	\text{\ \textbrokenbar\ }
% 	\left\langle z\right\rangle_{B} ).  
% 	\end{equation}
% 	This primitive is done by using Beaver's triplet technique(see \cite{beaver1991efficient} for more details) .
% 	%are proposed to simplify multiplication on secret shared inputs. 
% 	%Two random values are used to hide the computation inputs and their multiplication used together with public differences to restore the correct multiplication result\cite{beaver1991efficient}. 
% 	We denote the computation as $\left\langle z\right\rangle=\left\langle x\right\rangle \cdot \left\langle y\right\rangle$ for simplicity.
	
% 	%\item 
	
% 	\textbf{SDIV}: Divide two \textit{SS} variables and get a new \textit{SS} variable of their original quotient as the result, having $z=x / y$:
% 	\begin{equation}
% 	\textit{SDIV}: (\left\langle x\right\rangle_{A}, \left\langle y\right\rangle_{A} \text{\ \textbrokenbar\ }
% 	\left\langle x\right\rangle_{B}, \left\langle y\right\rangle_{B}
% 	)\mapsto( \left\langle z\right\rangle_{A} 
% 	\text{\ \textbrokenbar\ }
% 	\left\langle z\right\rangle_{B} ).  
% 	\end{equation}
% 	This primitive is implemented with the numerical optimization algorithms. The functional iteration methods are expanded
% 	to secure division, e.g. Goldschmidt’s series expansion algorithm\cite{goldschmidt1964applications}. Then the division
% 	can be approximated and computed with the \textit{SMUL} \& \textit{SADD}. With proper initial approximation, the convergence
% 	is guaranteed. We denote the computation as $\left\langle z\right\rangle=  \left\langle x\right\rangle / \left\langle y\right\rangle$
% 	for simplicity.
	
% 	%\item 
	
% 	\textbf{SARGMAX}: Take a matrix of \textit{SS} variables as input and return the indexes of the variable with max original value:
% 	\begin{equation}
% 	\textit{SARGMAX}: (\left\lbrace \left\langle x\right\rangle_{A} \right\rbrace^{i,j}\text{\ \textbrokenbar\ }\left\lbrace \left\langle x\right\rangle_{B} \right\rbrace^{i,j} )  
% 	\mapsto \arg\max_{i, j}(\left\lbrace  x \right\rbrace^{i, j} ). 
% 	\end{equation}
% 	In practice, the indexes are \textit{SS} variables for the sake of security. In our algorithm, the output of \textbf{SARGMAX} is the permuted feature bucket indexes without leaking the order infomation. So we skip the reveal process and denote the computation as $(i,j)= \arg\max\limits_{i,j}( \left\lbrace \left\langle x\right\rangle \right\rbrace^{i,j} ) $ for simplicity.
	
%\end{itemize}


\subsection{Secret Sharing Protocols}\label{secprot}
In general, the GMW protocol~\cite{goldreich2019play,goldreich2007foundations} shares a $l$-bit value $x$ additively in the ring $\mathbb{Z}_{2^{l}}$  as the sum of two values, where $l$ is the length of the numbers and $2^l$ is the size of the computation finite field. With different $l$, GMW can work on both Boolean and Arithmetic circuits. 
%We adopt both types of circuits for different computation protocols. 
%
% This mechanism satisfies the nice additive homomorphism that \textit{Addition} and 	\textit{Scalar-Multiplication} can be executed  without any interaction. \ccc{cannot follow}
% %
% Further, it can be naturally generalized to more than two parties.
% GMW has two operations, i.e., \textit{Addition} and \textit{Scalar-Multiplication}, which can be executed without any interaction, and other operations which needs interactions during executions. 
We describe the necessary computation protocols below under the two-party setting. 
%
Note that these protocols can be naturally generalized to more than two parties.

\nosection{Sharing scheme} 
We denote a secretly shared value $x$ 
by angle brackets, i.e., $\langle x\rangle$. 
Specifically, it consists of two random shares, i.e., $\langle x\rangle_{0}$ and $\langle x\rangle_{1}$, which are physically distributed at parties $P_{0}$ and $P_{1}$, respectively. According to the definition of additive secret sharing,
we have $x = \langle x\rangle_{0}+\langle x\rangle_{1}~mod~2^l$. Note that we will omit $2^l$ for conciseness in the following formulas.
%and perform the computations with rational numbers using fixed-point representation \cite{mohassel2017secureml}.

\nosection{Initialization} 
$Init(x)$, transforming a private input at one party
%for vertical federated learning, data of one participant can be transformed 
into \textit{Secret Sharing} format among two parties. 
We take a private value $x$ of $P_{0}$ for example.
%Suppose that $P_{0}$ holds a private value $x$ and wants to share it. 
Firstly, $P_{0}$ chooses a random number $r \in \mathbb{Z}_{2^{l}}$ and sends it to $P_{1}$. Then $P_{0}$ sets its local share as $\langle x\rangle_{0}=x-r$. 
Meanwhile, $P_{1}$ finishes the computation by setting $\langle x\rangle_{1}=r$. The correctness is obvious since $\langle x\rangle_{0}+\langle x\rangle_{1}=x$. The random number $r$ guarantees privacy, as a mask of $x$, and reveals nothing to $P_{1}$. %Similarly, $P_{1}$ could generate random masks for its inputs and sends the masks to $P_{0}$.

\nosection{Reconstruction} 
$Rec(\langle x\rangle)$. After a batch of secure computations, the final result is obtained in secret sharing representation. To reconstruct it, two parties should exchange their local shares %(e.g. $P_{i}$ holds $\langle x\rangle_{i}$) 
and sum them up.

\nosection{Addition} $\langle z\rangle = \langle x\rangle + \langle y\rangle$. $P_{i}$ locally computes $\langle z\rangle_{i} = \langle x\rangle_{i} + \langle y\rangle_{i}$ ($i\in \{0,1\}$). 
%
Since $\langle z\rangle_{0}+\langle z\rangle_{1}=\langle x\rangle_{0}+\langle x\rangle_{1}+\langle y\rangle_{0}+\langle y\rangle_{1}=x+y$, $(\langle z\rangle_{0}, \langle z\rangle_{1})$ is a correct secret sharing pair of the sum $z$. Similarly, $Subtraction$ protocol can be implemented with local subtraction.

\begin{figure}[t]
	\centering
% 	\vskip -0.2in
	\includegraphics[width=0.4\textwidth]{pics/ss_eg.pdf}
		\vskip -0.1in
	\caption{Illustration of secret sharing addition.}\label{figsseg}
\vspace{-0.15in}
\end{figure}
	
We show an example in Figure \ref{figsseg} to better illustrate the idea of secret sharing and the above protocols. 
%
Two parties (A and B) hold two private values (3 and 5) separately, and want to jointly compute the sum without leaking out the original value. 
%
The parties first share their private inputs with the \textit{Initialization} protocol. For example, party A splits its value 3 randomly into 2 shares (2, 1) and holds one locally, i.e. number 2. 
%
Party B cannot infer the original value only with received share and has to guess the other share equiprobably within the finite field.
%From the perspective of party B, it has to guess the other share with even possibilities among all the numbers in the finite field and cannot shrink the search space. 
Thus the private input is protected by the share randomness.
%
%Similarly, the private input 5 of Party B is securely distributed to both parties by secret sharing. 
Then two parties execute \textit{Addition} protocol by adding their local shares %of the augend and the addend
(e.g., $2+4=6$). 
%
At this point, the result shares (6, 2) make up the \textit{Secret Sharing} representation of the sum and the computation is secure. After the computation, the parties obtain the result by calling the $Reconstruction$ protocol.
%After the computation, if the parties want to obtain the result, they need to get the missing share from the opposite party (e.g. party A will get number 2 from party B). By summing up the shares, both parties can reconstruct the result ($6+2=8$). 
%
% Note that, secret sharing, as well as other multi-party computation techniques, protect the security in the computation process instead of computation result. 
% For example, party B can infer the input of party A as long as the correct sum is obtained. In this way, the private input is not revealed by the interactions and local computation but the result, as analyzed above. In practice, the computations are much complicated than a single addition and the private inputs cannot be inferred any more. There are a few necessary protocols besides the above ones.
% \ccc{this para. could be simplified}

\nosection{Scalar-multiplication} $\langle y\rangle=c \cdot \langle x\rangle$, where $c$ is the public scalar known to both parties.  $P_{i}$ locally computes $\langle y\rangle_{i}=c\cdot \langle x\rangle_{i}$ ($i\in \{0,1\}$). Then we have $\langle y\rangle_{0}+\langle y\rangle_{1}=c \cdot (\langle x\rangle_{0}+\langle x\rangle_{1})=c\cdot x$, and $(\langle y\rangle_{0}, \langle y\rangle_{1})$ is a correct secret sharing pair of the product $y$. 

\nosection{Multiplication} 
$\langle z\rangle=\langle x\rangle \cdot \langle y\rangle$. Because GMW scheme holds the additive homomorphism~\cite{evans2017pragmatic}, it can integrate with the Beaver-triplet approach to achieve an efficient online computation~\cite{beaver1991efficient}. 
A Beaver-triplet contains three secret shared values $( \langle a\rangle, \langle b\rangle, \langle c\rangle)$, where a and b are uniformly random values and $c = a\cdot b$. Then the parties compute $\langle e\rangle=\langle x\rangle-\langle a\rangle$ and $\langle f\rangle=\langle y\rangle-\langle b\rangle$ with $Subtraction$ protocol. In this way, $x$ and $y$ are securely masked by random values. $e$ and $f$ can be reconstructed without leakage. $P_{i}$ finishes the computation by computing locally $\langle z\rangle_{i}=-i\cdot e\cdot f+f\cdot \langle x\rangle_{i}+e\cdot \langle y\rangle_{i}+\langle c\rangle_{i}$.
% \begin{equation}
% \begin{split}
% \label{eqbeaver}
% xy&=(x-a+a)(y-b+b)\\
% &=(x-a)(y-b)+(x-a)b+a(y-b)+ab \\
% \implies \langle z\rangle&=Rec(\langle x\rangle - \langle a\rangle)\cdot Rec(\langle y\rangle - \langle b\rangle)\\
% &\textcolor[rgb]{0,0.6875,0.3125}{\boldsymbol{+}}\  Rec(\langle x\rangle - \langle a\rangle) \textcolor[rgb]{0,0.6875,0.9375}{\boldsymbol{\cdot} \langle b\rangle} \\
% &\textcolor[rgb]{0,0.6875,0.3125}{\boldsymbol{+}}\ Rec(\langle y\rangle - \langle b\rangle)  \textcolor[rgb]{0,0.6875,0.9375}{\boldsymbol{\cdot} \langle a\rangle}  \\
% &\textcolor[rgb]{0,0.6875,0.3125}{\boldsymbol{+}}\ \langle c\rangle.
% \end{split}
% \end{equation}
% Equation (\ref{eqbeaver}) explains the online computation process of multiplication. Two parties reconstruct $(x-a)$ and $(y-b)$  as public numbers at first. Because $x$ and $y$ are masked by random numbers $a$ and $b$ respectively, reconstructing the subtraction results leaks no private. 
%
% With the reconstructed numbers, the multiplication turns into two %\textcolor[rgb]{0,0.6875,0.9375}{Scalar-Multiplication} 
% \textit{Scalar-Multiplication}
% and three %\textcolor[rgb]{0,0.6875,0.3125}{Additions},
% \textit{Additions},
% which are locally computed. As for the first term, computing the product of the reconstructed numbers is a public multiplication, which can be executed on either side. 


% Since the triples are irrelevant to inputs $x$ and $y$, they can be mass-produced before the computation starts, i.e. the so-called \textit{offline process}. In our setting, this preparation is easily done with the help of a third-party server. %With Addition and Multiplication, non-linear functions could be approximated by Taylor expansion. 

Due to the fixed-point representation, a truncation is required as the postprocessing after each \textit{Multiplication}.
We adopt the efficient proposal in \cite{mohassel2017secureml}, which truncates the product shares independently. It has been proven that, with high probability, the reconstructed product is at most 1 bit off in the least significant position of the fractional part. This small truncation error is generally tolerable for machine learning applications with sufficient fractional bits. 

\nosection{Division} 
$\langle z\rangle=\langle x\rangle / \langle y\rangle$. We apply the Goldschmidt’s series expansion \cite{goldschmidt1964applications} and execute this numerical optimization algorithm with \textit{Addition} and \textit{Multiplication}. Following the work in \cite{catrina2010secure}, secure division offers sufficient accuracy with linear-approximated initialization and two computation iterations.

\nosection{Sigmoid} 
Classical sigmoid approximations includes Taylor expansion \cite{kim2018secure} and piece-wise approximation~\cite{mohassel2017secureml}. Taylor expansion explodes with large argument number which is a common case in large-scale training tasks. Piece-wise approximation faces the problem of precision loss, which is critical for the model accuracy. As an alternative, we apply $f(x)=\frac{0.5x}{1+|x|}+0.5$ to obtain a better approximation.
% \begin{equation}
% f(x)=\frac{0.5x}{1+|x|}+0.5.
% \label{eqnsig}
% \end{equation}

\nosection{Argmax} 
We first introduce the Boolean sharing \cite{demmler2015aby} to implement the \textit{Comparison} protocol, which enables bit decomposition of the subtraction of two numbers. In this way, we can get the sign of the subtraction which indicates the comparison result. Then, tree-reduction algorithm \cite{mohassel2020practical} computes \textit{Argmax} by partitioning the input into two halves and reduces the number of comparisons by half in each round.

\begin{algorithm}[t] 
	\begin{algorithmic}[1]  
		\caption{Training Algorithm of XGB}
		\label{alg:trainxgb}  
		\Function {TrainXGB}{$ X, Y, T, N$}
		\State $f_{0}=ComputeBaseScore(Y)$
		\State $model=[f_{0}]$  
		\For{$t=1,2,...,T$}
		\State $f_{t}=InitTree()$
		\State $P=PredictScore(X, model)$
		\State $\hat{Y}=Sigmoid(P)$
		\State $G_{t-1}=ComputeGradient(Y, \hat{Y})$
		\State $H_{t-1}=ComputeHessian(Y, \hat{Y})$
		\For{$n=1,2,...,N$}
		\If{n is a leaf}
		\State $w=ComputeWeight(G_{t-1}, H_{t-1}, f_{t}, n)$
		\State $f_{t}.SetWeight(w, n)$
		\Else
		\State $SG, SH=SumGradients(X, G_{t-1}, H_{t-1}, f_{t}, n)$
		\State $GA=ComputeGain(SG, SH)$
		\State $index=Argmax(GA)$
		\State $feat, val=RecSplitInfo(index)$
		\State $f_{t}.SetSplit(feat, val, n)$
		\State $f_{t}.SplitNode(feat, val)$
		\EndIf
		\EndFor
		\State $model.append(f_{t})$
		\EndFor
		\State \Return $model$
		\EndFunction
	\end{algorithmic}  
\end{algorithm}


==> HESS-XGB (2)/proof.tex <==
\appendix
\section{Security Proof}\label{proof}
\subsection{SumBucket based on SS}\label{proof-ss}

% \begin{small}
% \begin{tcolorbox}[colback=white,arc=0pt,outer arc=0pt,boxrule=0.7pt,enhanced,breakable,fontupper=\linespread{.8}\selectfont]
% \textbf{Functionality of SumBucket based on SS $\mathcal{F}_{\mathsf{SSSumBucket}}$}\\
%     \\
%     \textbf{Inputs:}
%     \begin{itemize}
%     	\item $\mathcal{A}$ inputs shares $\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M$, and $X_A,V_A$;
%         \item $\mathcal{B}$ inputs shares $\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M$, and $X_B,V_B$;.
%     \end{itemize}
%     \textbf{Outputs:}
%     \begin{itemize}
%         \item $\mathcal{A}$ outputs $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$;
%         \item $\mathcal{B}$ outputs $\{\langle bg \rangle_B\}^{j,k},\{\langle bh \rangle_B\}^{j,k}$.
%     \end{itemize}
% \end{tcolorbox}
% \end{small}



% \paragraph{Security Proof} We show that \textbf{Algorithm 4} is secure against semi-honest adversaries. Formally, we have the following theorem.

\begin{theorem}
	Assume that $\mathcal{F}_{\mathsf{N2S}}$ and $\mathcal{F}_{\mathsf{SMUL}}$ are secure primitives. Then, \textbf{Algorithm \ref{alg:ssbuck}} (denoted as $\pi_4$) is secure against semi-honest adversaries in $\mathcal{F}_{\mathsf{N2S}},\mathcal{F}_{\mathsf{SMUL}}$-hybrid model, as in \textbf{Definition 4.1}.
\end{theorem}





\begin{proof}
	We begin by proving the correctness of \textbf{Algorithm \ref{alg:ssbuck}}, i.e., we prove that $\{\langle bg \rangle_A\}^{j,k} + \{\langle bg \rangle_B\}^{j,k}$ is equal to $\Sigma_i\{ s_{jk}\}^i\cdot \{ g \}^i$, and $\{\langle bh \rangle_A\}^{j,k}+\{\langle bh \rangle_B\}^{j,k}$ is equal to $\Sigma_i\{ s_{jk}\}^i\cdot \{ h \}^i$.
	
	From the protocol execution, we know that $\{\langle bg \rangle\}^{j,k}=\Sigma_i\{\langle s_{jk}\rangle\}^i\cdot \{\langle g \rangle\}^i$. We denote $\{\langle s_{jk}\rangle\}^i\cdot \{\langle g \rangle\}^i$ as $\{\langle p \rangle\}^i$, and according to functionality $\mathcal{F}_{\mathsf{SMUL}}$, we have $\{ s_{jk}\}^i\cdot \{ g \}^i=\{ p \}^i$ and $\{\langle p \rangle_A\}^i+\{\langle p \rangle_B\}^i=\{ p \}^i$.
	
	Therefore, we have the following equation,
	\begin{equation}
		\begin{aligned}\nonumber
		\{\langle bg \rangle_A\}^{j,k}+\{\langle bg \rangle_B\}^{j,k}&=\Sigma_i\{\langle p \rangle_A\}^i+\Sigma_i\{\langle p \rangle_B\}^i\\
		&=\Sigma_i\{ p \}^i\\
		&=\Sigma_i\{ s_{jk}\}^i\cdot \{ g \}^i
		\end{aligned}
	\end{equation}
		
	Similarly, we have $\{\langle bh \rangle_A\}^{j,k}+\{\langle bh \rangle_B\}^{j,k}=\Sigma_i\{ s_{jk}\}^i\cdot \{ h \}^i$.
	
	This proves the correctness of \textbf{Algorithm \ref{alg:ssbuck}}. 
	
	We now prove that we can construct two simulators $\mathcal{S}_{\mathcal{A}}$ and $\mathcal{S}_{\mathcal{B}}$, such that
	\begin{eqnarray}
		\begin{aligned}
		&\{\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa} \label{eqn5}\\
		&\cong\{\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa},
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}
		\begin{aligned}
		&\{\mathcal{S}_{\mathcal{B}}(1^\kappa,\textsf{Input}_B,\{\langle bg \rangle_B\}^{j,k},\{\langle bh \rangle_B\}^{j,k})\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa}\\
		&\cong\{\mathsf{view}_{\mathcal{B}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa}, 
		\end{aligned}
	\end{eqnarray}
	where $\mathsf{view}_{\mathcal{A}}^{\pi_4}$ and $\mathsf{view}_{\mathcal{B}}^{\pi_4}$ denote the views of $\mathcal{A}$ and $\mathcal{B}$, respectively, while $\textsf{Input}_A=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,X_A,V_A)$ and $\textsf{Input}_B=(\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M,X_B,V_B)$ denote the inputs of $\mathcal{A}$ and $\mathcal{B}$, respectively.
	
	We then prove the above equations for a corrupted $\mathcal{A}$.
	
	\paragraph{Corrupted $\mathcal{A}$} 
	%In this case, we construct a probabilistic polynomial-time simulator $\mathcal{S}_{\mathcal{A}}$ that, when given the security parameter $\kappa$, $\mathcal{A}$'s input $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M$, $X_A,V_A)$ and output $(\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$, can simulate the view of $\mathcal{A}$ in the protocol execution. To this end, we first analyze $\mathcal{A}$'s view $\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ in \textbf{Algorithm 4}. 
	In \textbf{Algorithm \ref{alg:ssbuck}}, the messages obtained by $\mathcal{A}$ are consisted of two parts. The first part is from the functionality $\mathcal{F}_{\mathsf{N2S}}$, i.e., $\{\langle s_{jk}\rangle_A\}^i$; the second part is from the functionality $\mathcal{F}_{\mathsf{SMUL}}$, i.e., $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$. 
	Therefore, $\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ consists of $\mathcal{A}$'s input $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A)$, the randomness $r_{\mathcal{A}}$, and the shares $(\{\langle s_{jk}\rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$.
	
	
	Given $\kappa$, $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A)$ and $(\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$, $\mathcal{S}_{\mathcal{A}}$ generates a simulation of $\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ as follows. 
	
	\begin{itemize}
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{N2S}}$, randomly generates $\{\langle s_{jk}'\rangle_A\}^i$, and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{N2S}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ outputs $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$ to simulate the functionality $\mathcal{F}_{\mathsf{SMUL}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ generates a simulation by outputting $(\{\langle g \rangle_A\}^i_M$, $\{\langle h \rangle_A\}^i_M$, $X_A$, $V_A$, $r_{\mathcal{A}}$,$\{\langle s_{jk}'\rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$.
	\end{itemize}
	
	Therefore, we have the following two equations:
	\begin{small}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A,r_{\mathcal{A}},\{\langle s_{jk}\rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}),
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A,r_{\mathcal{A}},\{\langle s_{jk}'\rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}). 
		\end{aligned}
	\end{eqnarray}
	\end{small}
		
	We note that the probability distributions of $\mathcal{A}$'s view and $\mathcal{S}_{\mathcal{A}}$'s output are identical.
	We thereby claim that Equation (\ref{eqn5}) holds.
	
	This completes the proof in the case of corrupted $\mathcal{A}$.
	Similarly, We can construct a simulator in the case of corrupted $\mathcal{B}$.
	In summary, \textbf{Algorithm \ref{alg:ssbuck}} securely computes $\mathcal{F}_{\mathsf{SSSumBucket}}$ against semi-honest adversaries in $\mathcal{F}_{\mathsf{N2S}},\mathcal{F}_{\mathsf{SMUL}}$-hybrid model.

	
\end{proof}







\subsection{SumBucket based on HESS}\label{proof-hess}

% \begin{small}
% \begin{tcolorbox}[colback=white,arc=0pt,outer arc=0pt,boxrule=0.7pt,enhanced,breakable,fontupper=\linespread{.8}\selectfont]
% \textbf{Functionality of SumBucket based on HESS $\mathcal{F}_{\mathsf{HESSSumBucket}}$}\\
%     \\
%     \textbf{Inputs:}
%     \begin{itemize}
%     	\item $\mathcal{A}$ inputs shares $\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M$, and $X_A,V_A$;
%         \item $\mathcal{B}$ inputs shares $\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M$, and $X_B,V_B$;.
%     \end{itemize}
%     \textbf{Outputs:}
%     \begin{itemize}
%         \item $\mathcal{A}$ outputs $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$;
%         \item $\mathcal{B}$ outputs $\{\langle bg \rangle_B\}^{j,k},\{\langle bh \rangle_B\}^{j,k}$.
%     \end{itemize}
% \end{tcolorbox}
% \end{small}



% \paragraph{Security Proof} We show that \textbf{Algorithm 5} is secure against semi-honest adversaries. Formally, we have the following theorem.

\begin{theorem}
	Assume that the additively homomorphic cryptosystem $\Pi=(\textsf{KeyGen}$, $ \textsf{Enc}$, $\textsf{Dec})$ is indistinguishable under chosen-plaintext attacks, $\mathcal{F}_{\mathsf{S2H}}$ and $\mathcal{F}_{\mathsf{H2S}}$ are secure primitives as mentioned before. Then, \textbf{Algorithm \ref{alg:hessbuck}} (denoted as $\pi_5$) is secure against semi-honest adversaries in $\mathcal{F}_{\mathsf{S2H}},\mathcal{F}_{\mathsf{H2S}}$-hybrid model, as in \textbf{Definition 4.1}.
\end{theorem}





\begin{proof}
	We begin by proving the correctness of \textbf{Algorithm \ref{alg:hessbuck}}, \ie we prove that $\{\langle bg \rangle_A\}^{j,k} + \{\langle bg \rangle_B\}^{j,k}$ is equal to $\Sigma_i\{ s_{jk}\}^i\cdot \{ g \}^i$, and $\{\langle bh \rangle_A\}^{j,k}+\{\langle bh \rangle_B\}^{j,k}$ is equal to $\Sigma_i\{ s_{jk}\}^i\cdot \{ h \}^i$.
	
	From the protocol execution, we know that the decryption of $\{[bg]_P\}^{j,k}$ is equal to $\{\langle bg \rangle_A\}^{j,k} + \{\langle bg \rangle_B\}^{j,k}$, where $\{[bg]_P\}^{j,k}=\Sigma_i\{s_{jk}\}^i\cdot\{[g]_{P}\}^i$. Therefore, we have $\{\langle bg \rangle_A\}^{j,k} + \{\langle bg \rangle_B\}^{j,k}=\Sigma_i\{ s_{jk}\}^i\cdot \{ g \}^i$. 
	Similarly, we have $\{\langle bh \rangle_A\}^{j,k}+\{\langle bh \rangle_B\}^{j,k}=\Sigma_i\{ s_{jk}\}^i\cdot \{ h \}^i$. This proves the correctness of \textbf{Algorithm \ref{alg:hessbuck}}. 
	
	In order to prove the security, we now construct the simulator $\mathcal{S}_{\mathcal{A}}$ and omit the symmetric construction for Corrupted $\mathcal{B}$.
	
	In \textbf{Algorithm \ref{alg:hessbuck}}, the messages obtained by $\mathcal{A}$ are consisted of two parts. The first part is from the functionality $\mathcal{F}_{\mathsf{S2H}}$, \ie $\{[g]_B\}^i,\{[h]_B\}^i$, and the second part is from the functionality $\mathcal{F}_{\mathsf{H2S}}$, \ie $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$. 
	Therefore, $\mathsf{view}_{\mathcal{A}}^{\pi_5}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ consists of $\mathcal{A}$'s input $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A)$, the randomness $r_{\mathcal{A}}$, and the messages $(\{[g]_B\}^i,\{[h]_B\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$.
	
	
	Given $\kappa$, $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A)$ and $(\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$, $\mathcal{S}_{\mathcal{A}}$ generates a simulation as follows. 
	
	\begin{itemize}
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{S2H}}$, randomly selects $\{g'\}^i$ and $\{h'\}^i$, encrypts them using $\mathcal{B}$'s public key $PK_B$ and obtains $\{[g']_B\}^i,\{[h']_B\}^i$. It takes $\{[g']_B\}^i,\{[h']_B\}^i$ as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{S2H}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{H2S}}$, takes $\{\langle bg \rangle_A\}^{j,k}$ and $\{\langle bh \rangle_A\}^{j,k}$ as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{H2S}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ generates a simulation of $\mathsf{view}_{\mathcal{A}}^{\pi_5}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ by outputting $(\{\langle g \rangle_A\}^i_M$, $\{\langle h \rangle_A\}^i_M$, $X_A$, $V_A$, $r_{\mathcal{A}}$,$\{[g']_B\}^i,\{[h']_B\}^i,$ $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$.
	\end{itemize}
	
	Therefore, we have the following two equations:
	\begin{small}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathsf{view}_{\mathcal{A}}^{\pi_5}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,X_A,V_A,r_{\mathcal{A}},\{[g]_B\}^i,\{[h]_B\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}),
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,X_A,V_A,r_{\mathcal{A}},\{[g']_B\}^i,\{[h']_B\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}). 
		\end{aligned}
	\end{eqnarray}
	\end{small}
		
	We note that as the additively homomorphic cryptosystem $\Pi$ is indistinguishable under chosen-plaintext attacks, the probability distributions of $\mathcal{A}$'s view and $\mathcal{S}_{\mathcal{A}}$'s output are computationally indistinguishable. 
	This completes the proof in the case of corrupted $\mathcal{A}$.
	
	In summary, \textbf{Algorithm \ref{alg:hessbuck}} securely computes $\mathcal{F}_{\mathsf{HESSSumBucket}}$ against semi-honest adversaries in $\mathcal{F}_{\mathsf{S2H}},\mathcal{F}_{\mathsf{H2S}}$-hybrid model.

	
\end{proof}







\subsection{Splitnode based on SS}\label{proof-splitnode}

% \begin{small}
% \begin{tcolorbox}[colback=white,arc=0pt,outer arc=0pt,boxrule=0.7pt,enhanced,breakable,fontupper=\linespread{.8}\selectfont]
% \textbf{Functionality of Splitnode based on SS $\mathcal{F}_{\mathsf{SSSplitNode}}$}\\
%     \\
%     \textbf{Inputs:}
%     \begin{itemize}
%     	\item $\mathcal{A}$ inputs shares $\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M$, and $X_A,V_A$;
%         \item $\mathcal{B}$ inputs shares $\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M,\{\langle s \rangle_B\}^i_M$, and $X_B,V_B$;.
%     \end{itemize}
%     \textbf{Outputs:}
%     \begin{itemize}
%         \item $\mathcal{A}$ outputs $\{\langle p \rangle_A\}^i_M$;
%         \item $\mathcal{B}$ outputs $\{\langle p \rangle_B\}^i_M$.
%     \end{itemize}
% \end{tcolorbox}
% \end{small}



% \paragraph{Security Proof} We show that \textbf{Algorithm 3} is secure against semi-honest adversaries. Formally, we have the following theorem.

\begin{theorem}
	Assume that $\mathcal{F}_{\mathsf{N2S}}$, $\mathcal{F}_{\mathsf{SMUL}}$, $\mathcal{F}_{\mathsf{SDIV}}$, $\mathcal{F}_{\mathsf{SSSumbucket}}$ and $\mathcal{F}_{\mathsf{SMAX}}$ are secure primitives as defined above. Then, \textbf{Algorithm \ref{alg:sssplit}} (denoted as $\pi_3$) is secure against semi-honest adversaries in $\mathcal{F}_{\mathsf{N2S}},\mathcal{F}_{\mathsf{SMUL}},$ $\mathcal{F}_{\mathsf{SDIV}},\mathcal{F}_{\mathsf{SSSumBucket}},\mathcal{F}_{\mathsf{SMAX}}$-hybrid model, as in \textbf{Definition 4.1}.
\end{theorem}





\begin{proof}
	We prove that we can construct two simulators $\mathcal{S}_{\mathcal{A}}$ and $\mathcal{S}_{\mathcal{B}}$, such that
	\begin{eqnarray}
		\begin{aligned}
		&\{\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle p \rangle_A\}^i_M)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa} \label{eqn6}\\
		&\cong\{\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa},
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}
		\begin{aligned}
		&\{\mathcal{S}_{\mathcal{B}}(1^\kappa,\textsf{Input}_B,\{\langle p \rangle_B\}^i_M)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa}\\
		&\cong\{\mathsf{view}_{\mathcal{B}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa}, 
		\end{aligned}
	\end{eqnarray}
	where $\mathsf{view}_{\mathcal{A}}^{\pi_3}$ and $\mathsf{view}_{\mathcal{B}}^{\pi_3}$ denote the views of $\mathcal{A}$ and $\mathcal{B}$, respectively, while $\textsf{Input}_A=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M,X_A,V_A)$ and $\textsf{Input}_B=(\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M$, $\{\langle s \rangle_B\}^i_M,X_B,V_B)$ denote the inputs of $\mathcal{A}$ and $\mathcal{B}$, respectively. We prove the above equations for a corrupted $\mathcal{A}$ and omit similar construction for a corrupted $\mathcal{B}$.
	
	Without loss of generality, we assume that the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$ happens only once in \textbf{Algorithm \ref{alg:sssplit}}. That is, we assume that for the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$ at line 48 in \textbf{Algorithm \ref{alg:sssplit}}, $\mathcal{F}_{\mathsf{SSSplitNode}}$ directly runs lines 4-10 and returns $\{\langle y \rangle\}^i$ as $\{\langle p_l \rangle\}^i$. For the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$ at line 49 in \textbf{Algorithm \ref{alg:sssplit}}, $\mathcal{F}_{\mathsf{SSSplitNode}}$ directly runs lines 4-10 and returns $\{\langle y \rangle\}^i$ as $\{\langle p_r \rangle\}^i$. We note that this assumption is just for a simpler and clearer description of the security proof, and will not lead to any security issues during the simulation of corrupted $\mathcal{A}$ or corrupted $\mathcal{B}$.
	
	\paragraph{Corrupted $\mathcal{A}$}In \textbf{Algorithm \ref{alg:sssplit}}, the messages obtained by $\mathcal{A}$ are consisted of five parts. The first part is from the functionality $\mathcal{F}_{\mathsf{N2S}}$, \ie $\langle sg_{l}\rangle_A,\langle sh_{l}\rangle_A$ and $\{\langle s_l \rangle_A\}^i,\{\langle s_r \rangle_A\}^i$; the second part is from the functionality $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$, \ie $\langle cgain \rangle_A$, $\{\langle gain \rangle_A\}^{j,k}$, $\{\langle g_l \rangle_A\}^i,\{\langle h_l \rangle_A\}^i,\{\langle g_r \rangle_A\}^i,\{\langle h_r \rangle_A\}^i$, and the new shares $\{\langle s'_l \rangle_A\}^i,$ $\{\langle s'_r \rangle_A\}^i$; the third part is from the functionality $\mathcal{F}_{\mathsf{SSSumBucket}}$, \ie $\{\langle bg \rangle_A\}^{j,k},$ $\{\langle bh \rangle_A\}^{j,k}$; the forth part is from the functionality $\mathcal{F}_{\mathsf{SMAX}}$, \ie the indices $j_{best},k_{best}$; and the fifth part is from the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$. To be specific, the messages in this part are actually from the functionality $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$, \ie $node.\langle weight_1\rangle_A,$ $\{\langle p_l \rangle_A\}^i$ and $node.\langle weight_2\rangle_A, \{\langle p_r \rangle_A\}^i$. 
	
	Therefore, $\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ consists of $\mathcal{A}$'s input $(\{\langle g \rangle_A\}^i_M$, $\{\langle h \rangle_A\}^i_M$, $\{\langle s \rangle_A\}^i_M$, $X_A$, $V_A)$, the randomness $r_{\mathcal{A}}$, and the above mentioned indices and shares.
	
	
	Given $\kappa$, $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M, X_A,V_A)$ and $\{\langle p \rangle_A\}^i_M$, $\mathcal{S}_{\mathcal{A}}$ generates a simulation of $\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ as follows. 
	
	\begin{itemize}
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{N2S}}$, randomly generates $\langle sg'_{l}\rangle_A,\langle sh'_{l}\rangle_A$ and $\{\langle s''_l \rangle_A\}^i,\{\langle s''_r \rangle_A\}^i$, and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{N2S}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$, randomly generates $\langle cgain' \rangle_A$,
		$\{\langle gain' \rangle_A\}^{j,k}$,
		$\{\langle g'_l \rangle_A\}^i$,
		$\{\langle h'_l \rangle_A\}^i$,
		$\{\langle g'_r \rangle_A\}^i$,
		$\{\langle h'_r \rangle_A\}^i$, 
		$\{\langle s'''_l \rangle_A\}^i$,
		$\{\langle s'''_r \rangle_A\}^i$ and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{SSSumBucket}}$, randomly generates $\{\langle bg' \rangle_A\}^{j,k}$, $\{\langle bh' \rangle_A\}^{j,k}$, and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{SSSumBucket}}$.
		\item {$\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{SMAX}}$, randomly generates $j'_{best},k'_{best}$, and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{SMAX}}$.}
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$. Specifically, during the recursion, $\mathcal{S}_{\mathcal{A}}$ needs to simulate the functionality $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$ again as follows. It randomly generates $node.\langle weight'_1\rangle_A, node.\langle weight'_2\rangle_A, \{\langle p'_l \rangle_A\}^i$, computes $\{\langle p'_r \rangle_A\}^i=\{\langle p \rangle_A\}^i-\{\langle p'_l \rangle_A\}^i$, and takes them as the output for $\mathcal{A}$ in the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ generates a simulation of $\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ by outputting the inputs $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M, X_A,V_A)$, the randomness $r_{\mathcal{A}}$, and all the simulated indices and shares above.
	\end{itemize}
	
	Therefore, we have the following two equations:
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M, X_A,V_A,r_{\mathcal{A}},\langle sg_{l}\rangle_A,\langle sh_{l}\rangle_A,\{\langle s_l \rangle_A\}^i,\\
		&\{\langle s_r \rangle_A\}^i,\langle cgain \rangle_A,\{\langle gain \rangle_A\}^{j,k},\{\langle g_l \rangle_A\}^i,\{\langle h_l \rangle_A\}^i,\{\langle g_r \rangle_A\}^i,\\
		&\{\langle h_r \rangle_A\}^i,\{\langle s'_l \rangle_A\}^i,\{\langle s'_r \rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k},j_{best},k_{best},\\
		&node.\langle weight_1\rangle_A,node.\langle weight_2\rangle_A,\{\langle p_l \rangle_A\}^i,\{\langle p_r \rangle_A\}^i),
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle p \rangle_A\}^i_M)\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M, X_A,V_A,r_{\mathcal{A}},\langle sg'_{l}\rangle_A,\langle sh'_{l}\rangle_A,\{\langle s''_l \rangle_A\}^i,\\
		&\{\langle s''_r \rangle_A\}^i,\langle cgain' \rangle_A,\{\langle gain' \rangle_A\}^{j,k},\{\langle g'_l \rangle_A\}^i,\{\langle h'_l \rangle_A\}^i,\{\langle g'_r \rangle_A\}^i,\\
		&\{\langle h'_r \rangle_A\}^i,\{\langle s'''_l \rangle_A\}^i,\{\langle s'''_r \rangle_A\}^i,\{\langle bg' \rangle_A\}^{j,k},\{\langle bh' \rangle_A\}^{j,k},j'_{best},k'_{best},\\
		&node.\langle weight'_1\rangle_A, node.\langle weight'_2\rangle_A,\{\langle p'_l \rangle_A\}^i,\{\langle p'_r \rangle_A\}^i). 
		\end{aligned}
	\end{eqnarray}
	
	
	
		
	We note that the probability distributions of $\mathcal{A}$'s view and $\mathcal{S}_{\mathcal{A}}$'s output are identical.
	We thereby claim that Equation (\ref{eqn6}) holds. This completes the proof in the case of corrupted $\mathcal{A}$. 
	
	After similar construction for a corrupted $\mathcal{B}$, we conclude that \textbf{Algorithm \ref{alg:sssplit}} securely computes $\mathcal{F}_{\mathsf{SSSplitNode}}$ against semi-honest adversaries in $\mathcal{F}_{\mathsf{N2S}},\mathcal{F}_{\mathsf{SMUL}},\mathcal{F}_{\mathsf{SDIV}},\mathcal{F}_{\mathsf{SSSumBucket}},\mathcal{F}_{\mathsf{SMAX}}$-hybrid model.

\end{proof}

==> HESS-XGB (2)/relatedwork.tex <==
\section{Related Work}
% In this section, we review related literature on  cryptography based secure decision tree and privacy preserving gradient tree boosting.%, and both of them have training and inference (prediction) methods, as summarized in \cite{chatel2021sok}. 
% a survey paper on privacy-preserving tree based model \cite{chatel2021sok}

\subsection{Secure Decision Tree}
% Existing works on cryptography based secure decision tree come in two types, i.e., secure training and secure prediction. 

\nosection{Training}
Most secure tree building (training) approaches choose the Iterative Dichotomizer 3 (ID3) \cite{quinlan1986induction} algorithm to build decision trees. 
For example, the first secure decision tree was proposed by Lindell \& Pinkas \cite{lindell2000privacy},  where they assume data are horizontally partitioned over two parties and their protocol is based on oblivious transfer \cite{naor1999oblivious} and Yao's garbled circuit  \cite{yao1986generate}. 
% The authors in \cite{xiao2005privacy,samet2008privacy} used homomorphic encryption to create secure ID3 under data horizontally partitioned setting. 
Later on, Hoogh et al., proposed a secret sharing based secure ID3 protocol \cite{de2014practical} which is suitable for any number of participants who horizontally partition the dataset. 
Protocols in \cite{du2002building,wang2006classification} are for secure ID3 over vertically partitioned data, assuming that all parties have the class attribute. 
%\cite{vaidya2005privacy} where a secure set of protocols for vertically partitioned data over more than two parties is discussed without disclosing any additional information and where not all parties have the class attribute

\nosection{Prediction}
Another line of work is the secure prediction (scoring) of decision tree 
\cite{wu2016privately,de2017efficient,kiss2019sok}. 
They assume that there is a server who holds a decision tree and a client who provides private features. 
After the protocol, the client obtains the classification result, without learning any information about the tree beyond its size and the prediction output, and the server learns nothing about the client's input features \cite{kiss2019sok}. 
There are also several literature on securely evaluating ID3 over horizontally partitioned data for more than two parties by HE \cite{xiao2005privacy,samet2008privacy}. 

% In this paper, instead of focusing on secure ID3, we aim to build secure gradient tree boosting training and prediction algorithms, which are more effective but complicated than ID3. 

\subsection{Privacy Preserving Gradient Tree Boosting}

\nosection{Training}
Besides secure decision tree, there are also several researches on privacy preserving gradient tree boosting. 
For example, \cite{liu2019boosting} and \cite{li2019practical} proposed federated gradient boosting decision tree and federated XGB under horizontal federated learning setting, respectively. That is, they assume data samples with the same features are distributed horizontally among mobile devices or multiple parties. 
Meanwhile, the authors of \cite{fengy2019securegbm,cheng2019secureboost,tian2020federboost} proposed privacy preserving XGB for vertically partitioned data setting. 
They are the most similar work to ours in literature. 
However, the models in \cite{fengy2019securegbm,cheng2019secureboost} are not provable secure. As we described in Section \ref{intro}, intermediate information is revealed during model training procedure. 
What is more, the leaked information cannot be quantified, which may cause potential privacy leakage in practice \cite{weng2020privacy}. 
Besides, the model proposed in \cite{tian2020federboost} relies on differential privacy, which indicates a trade-off between privacy and utility. 
In contrast, in this paper, we present a provable and lossless secure XGB by leveraging secure multi-party computation techniques, including secret sharing, HE, and correlated randomness.

% multi-party vertical FedXGB \cite{xie2021efficient} \ccc{cannot tell main difference}


\nosection{Prediction}
There is also work on building secure XGB prediction models~\cite{meng2020privacy,chen2021fed}. 
For example, Meng and Feignebaum applied HE for secure XGB prediction under the same client-server mode as decision tree. 
%
Later on, Chen et al. proposed a HE based federated XGB inference for multiple parties \cite{chen2021fed}, which assumes that the tree structures are distributed among multiple parties.
%
In this paper, we propose to leverage secret sharing for secure tree prediction, which avoids time-consuming HE operations. 

==> HESS-XGB (2)/work.tex <==
\section{The proposed model}\label{secxgb}
% As the basis of the framework, we employ the additive secret sharing scheme and essential computation protocols, with which we can obtain a baseline secure model. By revisiting baseline model, we tackle the bottle neck with a novel building block(i.e. secret permutation) and propose two more efficient variants. The two variants are practically neck-and-neck, so we can choose a more appropriate one according to the specific computation performance and communication condition. Though we illustrate the models under 2-party setting, they are flexible to be extended for more participants.

In this section, we first present SS-XGB by leveraging secret sharing. We then propose HEP-XGB and CRP-XGB which improve the efficiency of SS-XGB by secure permutation. We finally propose a secure XGB prediction algorithm.  

%
%The two variants are practically neck-and-neck, so we can choose a more appropriate one according to the specific computation performance and communication condition. %Though we illustrate the models under 2-party setting, they are flexible to be extended for more participants. 
%\ccc{will move to later sec}



\subsection{SS-XGB}
%We first present a secure XGB training model, i.e., SS-XGB, by leveraging secret sharing technique. 
%

We start from the general XGB training in Algorithm \ref{alg:trainxgb} and later will turn it into a secure version with proper modifications. The inputs are a feature matrix $X$ and a label vector $Y$. As an additive model, XGB first makes an initial guess (line 2), followed by the predictions from the $T$ tree models as revisions (line 4-24), where $T$ is the number of trees. XGB simplifies the objective function with second-order Taylor approximation. Before each tree fitting process, the gradients are computed (line 8-9) with the up-to-date predictions (line 6-7). With the help of the gradients, the algorithm proceeds to split each node (line 10-22), where $N$ is the number of nodes. If we reach a leaf node, the associated weight is computed and stored in the model (line 11-13). Otherwise, we should enumerate all possible split candidates and 
compute the gradient sums of the containing instances in each split bucket (line 15). With the accumulated gradients and Equation (\ref{eqobj}), the feature and value with the max split gain are obtained (line 16-18). Then we update the split information in tree and split the instances into two child nodes (line 19-20). After traversing all the nodes, a new tree is built and appended to the model list (line 23).
In this way, the model is finally returned with a base score and $T$ trees.


Our proposed SS-XGB model remains unchanged as XGB except for the following adaptations:

\nosection{Hide source data} 
In order to protect the private inputs, the label $Y$ and the intermediate calculations, e.g., $G$, $H$, and $GA$ (line 16), are represented in secret sharing scheme. 
%
The computations are all replaced with the secure protocols described in Section \ref{secprot}. Following the paradigm of secret sharing, nothing but the output model will be revealed.

\begin{figure}[t]
	\centering
% 	\vspace{-0.15in}
	\includegraphics[width=0.32\textwidth]{pics/inst.pdf}
		\vskip -0.1in
	\caption{A toy data example.}\label{figinst}
% 		\vskip -0.05in
% \vspace{-0.2in}
\end{figure}

\nosection{Hide partial order} 
\textit{SumGradients} in Algorithm \ref{alg:trainxgb} turns out to be a major obstacle. We illustrate the problem with an example in Figure \ref{figinst}, where there are five instances in the data and the gradients are secret share values. Supposing that Party A holds a feature `Age', Figure \ref{figgsum} displays how to implement the \textit{SumGradients} directly, where we only consider the first-order gradient for convenience. 

\begin{figure}[t]
	\centering
% 	\vskip -0.15in
	\includegraphics[width=0.4\textwidth]{pics/gsum.pdf}
		\vskip -0.15in
	\caption{Unsecure \textit{SumGradients}.}\label{figgsum}
% 		\vskip -0.05in
% \vspace{-0.2in}
\end{figure}

Party A firstly sort the instances by feature `Age' and sums the gradients for all split candidates. For example, when the split condition is `Age<15', we should sum the gradients on the left side of the split point, i.e., $G_L=\langle g_1\rangle+\langle g_4\rangle$. According to the \textit{Addition} protocol in Section \ref{secprot}, Party A has to send the instance indexes to Party B, so that Party B is able to execute the local addition for correct instances.

However, in the process, Party A has to leak the partial order of feature `Age' to Party B after enumerating all the split points, i.e., 1 $\rightarrow$ 4 $\rightarrow$ 2 $\rightarrow$ 5 $\rightarrow$ 3. In order to hide the order, we introduce an indicator vector (vector $S$ in Figure \ref{figindi}). The instances to be accumulated is marked as 1 in $S$ by Party A and 0 otherwise. To preserve privacy, we also transform the indicator vector to secret shares. In this way, the sum of the gradients of the instances can be computed as the inner product of the indicator vector and the gradient vector, which can be securely computed by \textit{Addition} and \textit{Multiplication} protocols.

\begin{figure}[b]
	\centering
% \vspace{-0.2in}
	\includegraphics[width=0.35\textwidth]{pics/indicator.pdf}
		\vskip -0.15in
	\caption{Indicator-based secure \textit{SumGradients}.}\label{figindi}
% 		\vskip -0.05in
% \vspace{-0.2in}
\end{figure}

\nosection{Hide instance distribution} 
In XGB, the instances are partitioned into two child nodes after the best split point is determined. 
The instance distribution on nodes is also intermediate information, which should not be revealed. Again, we solve this with the indicator trick. We partition the instances by updating the gradients as secretly shared zeros for the unrelated instances. 

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{pics/dist.pdf}
		\vskip -0.1in
	\caption{Hide instance distribution.}\label{figdist}
% 		\vskip -0.05in
% \vspace{-0.2in}
\end{figure}

We illustrate why the secret partition works in Figure \ref{figdist}. 
%
Assuming `Age<15' is the best split point, we present how to update the gradient vector for left branch with $G_L$ in Figure \ref{figindi}. 
%
As we can see, the gradients for the 3 instances outside the left branch, i.e., in the right branch, are set as secret shared zeros. 
%
After it, we continue split the left branch with feature `Female' which is owned by Party B. 
%
After sorting the entire instances, the gradients on the left side of the split point can be computed. Because the invalid gradients are zeros, the accumulated gradients are equivalent to \textit{SumGradients} in the plaintext. 

With the above adaptations, two parties are able to jointly train secure XGB without any information leakage.


\subsection{HEP-XGB and CRP-XGB: Improving SS-XGB by Secure Permutation}\label{secsp}
% \subsection{Optimization: Secret Permutation}\label{secsp}
Although the above SS-XGB is secure, it could hardly handle large-scale datasets. 
%
Because we introduce redundant zeros and related computations, in the indicator trick, to confuse the adversary. 
%
Thus, the security is achieved at the cost of the heavy communication. Supposing that there are $M$ samples and $N$ features in the dataset, if we propose $K$ split values for each feature, the indicator matrix has $M$ rows and $(N\times K)$ columns. The gradient matrix has 2 rows (for first-order and second-order gradient respectively) and $M$ columns. Then the \textit{SumGradients} turns out to be a matrix multiplication of the gradient matrix and indicator matrix. The communication complexity is the sum of two matrices, i.e., $(MNK+2M)$, which is intolerable under real-world scenarios.

\begin{figure}[b]
	\centering
% \vspace{-0.2in}
	\includegraphics[width=0.25\textwidth]{pics/sp.pdf}
		\vskip -0.15in
	\caption{Secure permutation. }\label{figsp}
% 		\vskip -0.05in
% \vspace{-0.2in}
\end{figure}

The above bottleneck of SS-XGB motivates us to build a building block which could \textit{permute a secret shared vector with a given rank}. Taking the case in Figure \ref{figgsum} for instance, we have to sort the secret gradients with respect to feature `Age'. Party A generates the mapping permutation (1, 3, 5, 2, 4), which indicates the new indexes of the original elements. 

We display the functionality of the \textit{Secure Permutation} in Figure \ref{figsp}. This block permutes a secret shared vector $\langle X\rangle$ which has $n$ elements. 
The permutation is defined as a function $\pi$, which is a private input of Party A. The output $\langle Y\rangle$ is the secret shared vector that applies $\pi$ on vector $X$, i.e., $\langle Y\rangle=\langle\pi(X)\rangle$.
Next, we will propose two implementations for this building block and compare their performance theoretically.

\nosection{HE based permutation} 
The first method is based on Homomorphic Encryption (HE). Additive HE is a form of encryption with an additional evaluation capability for computing over encrypted data without access to the secret key. It is widely used for privacy-preserving outsourced computation \cite{fun2016survey}. The typical computation scheme is regarding one party as an encrypter and the other as a calculator. All computations are conducted by the calculator with ciphertexts. Because the calculator has no access to the secret key of encrypter, the original data and computations are secure. 

Intuitively, we can take advantage of HE scheme and take the permutation provider as the calculator. 
%
This can be done by mainly three steps. That is, (1) A and B transform the gradient vector from secret sharing scheme to HE scheme (\textit{S2H}), after which A holds a ciphertext vector, (2) A makes permutation on the ciphertext vector, and (3) A and B transform the permuted ciphertext vector from HE scheme to secret sharing scheme (\textit{H2S}). 
% In the above example, if the gradient vector is in the Homomorphic Encryption scheme, where Party A holds the cipertext vector and Party B holds the secret key. \ccc{why?}
% %
% Obviously, it is easier for A to permute the centralized cipertext vector than the distributed secret shares. So we can first transform gradient vector from Secret Sharing scheme to Homomorphic Encryption scheme and permute the cipertext vector. Then the permuted vector is transformed back to Secret Sharing scheme and carries on the training. 
In the following, we will elaborate how to securely transform between two schemes, i.e., \textit{S2H} and \textit{H2S}.

\textit{S2H}: 
we first represent the encrypted variable under HE scheme as $[x]_A$, where $x$ is the plaintext and $A$ denotes the encrypter. The \textit{S2H} protocol is described in Figure \ref{figs2h}, where Party A acts as the encrypter and provides the public key and Party B receives the encrypted share and outputs the sum in cipertext. In this process, Party B has no access to $SK_{A}$, and thus the security of the original value $x$ is guarantee by HE. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{pics/s2h.pdf}
% 		\vskip -0.15in
	\caption{S2H protocol.}\label{figs2h}
% 		\vskip -0.1in
\end{figure}

\textit{H2S}: 
We then explain the \textit{H2S} protocol step by step in Figure \ref{figh2s} whose correctness is obvious. As for the security, we look into it from two aspects.
On the one hand, $x$ is encrypted by $PK_{A}$ and party B cannot decrypt the ciphertext. On the other hand, Party A only gets ciphertext of the random share. 
Both parties have no access to the original value, thus the transformation is secure. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{pics/h2s.pdf}
% 		\vskip -0.15in
	\caption{H2S protocol.}\label{figh2s}
		\vskip -0.1in
\end{figure}

In order to reduce the communication, we accumulate the gradients under HE scheme and postpone the execution of \textit{H2S} protocol to the end of the \textit{SumGradients}. The communication is reduced to $2NK$, which is the size of the result matrix of \textit{SumGradients}.

\nosection{CR based permutation} 
The second method relies on Correlated Randomness (CR) under the secret share scheme. 
%
% Every functionality can be securely computed given access to an appropriate source of correlated randomness and no additional assumptions~\cite{ishai2013power}. 
%
The very first work on CR is the Beaver's multiplication triplet described in Section \ref{secprot}. The Beaver triples are input-independent random numbers and generated in the offline process. The three numbers in a triplet are correlated with each other. By utilizing this correlated randomness, the online process obtains significant speedup. 
%
There are also other types of CR, including garbled circuit correlation, OT correlation, OLE correlation, and one-time truth-tables~\cite{ishai2013power,damgaard2017tinytable,couteau2019note}.
Similarly, we can design specific CR for permutation function to achieve better performance.
%
We elaborate the CR based permutation protocol in Figure \ref{figsp_prot}, which mainly has four steps. 

\begin{figure}[t]
		\centering
		\includegraphics[width=0.5\textwidth]{pics/sp_prot.pdf}
% 		\vskip -0.1in
		\caption{CR based secure permutation.}\label{figsp_prot}
%		\vskip -0.1in
\end{figure}

In step 1, we employ the trust dealer to generate the triplet and dispatch the secret shares to both parties. We define the permutation triplet as ($\pi_{1}, \langle R\rangle, \langle  \pi_{1}(R)\rangle$), where $\pi_{1}$ is a random permutation order, $R$ is a vector with $n$ random numbers, and $\pi_{1}(R)$ denotes the result vector after permuting $R$ with $\pi_{1}$.  This step is independent of the XGB training process, and thus can be executed in the offline phase.

In step 2, we solve the transformation permutation function $\pi_{2}$, using the source permutation $\pi_{1}$ and the target permutation $\pi$. To do this, Party A performs this computation and sends $\pi_{2}$ to Party B. Note that, $\pi_{1}$ works as a random mask for $\pi$. Party B only receives the masked permutation $\pi_{2}$ and thus $\pi$ is securely hided.

In step 3, a $Reconstruction$ protocol is executed and reveals $(X-R)$ to Party A.
Similarly, the private vector $X$ is masked by the random vector $R$ in an element-wise manner. Thus, the $Reconstruction$ leaks out nothing about $X$.

In step 4, the parties locally compute the output shares. One can check the correctness as follows:
\begin{equation}
\begin{split}
Y &= \langle Y\rangle_{A}+\langle Y\rangle_{B} \\
&=\pi(X-R)+\pi_{2}[ \langle  \pi_{1}(R)\rangle_{A}+ \langle  \pi_{1}(R)\rangle_{B}] \\
&=\pi(X-R)+\pi_{2}[\pi_{1}(R)] \\
&=\pi(X-R)+\pi(R) =\pi(X).
\end{split}
\end{equation}

The secure permutation protocol is employed to sort the first-order and second-order gradients for XGB. The \textit{SumGradients} then accumulates the gradients with \textit{Addition} protocol, which contains only cheap local computations.
% From now on, we name the baseline approach as \textbf{SS-XGB}, which employs basic secret sharing protocols
%
We term the two optimized approaches, based on HE and CR secure permutation implementations, as \textbf{HEP-XGB} and \textbf{CRP-XGB} respectively.

\nosection{Complexity analysis} 
In general, SS-XGB and CRP-XGB only rely on secret sharing scheme, and thus they are computational efficient but have high communication cost. 
%
In contrast, since it is time-consuming for HE computations,  HEP-XGB is computationally intensive but with less communication overhead. 
%
All these approaches share the same algorithm flow except for \textit{SumGradients}, we summarize their time costs in this process below:
\begin{itemize}[leftmargin=*]
    \item SS-XGB: the communication is as analyzed in section \ref{secsp}, i.e., $MNK+2M\approx MNK$. 
    %Thus, the overall communication is about $2MNK$.
    \item CRP-XGB: to accumulate first and second order gradients, the online phase transmits a masked permutation and a revealing share, thus the total communication is $2MN$ plaintexts and $2MN$ shares. Compared with SS-XGB, CRP-XGB removes the bucket number ($K$) which is set to 33 by default. Therefore, not only the communication but also the memory are significantly reduced.
    \item HEP-XGB: the \textit{S2H} protocol is invoked for $2M$ times to transform gradients. And we need $2MN$ homomorphic additions to accumulate the encrypt gradients to belonging bucket, and $2KN$ invocations for \textit{H2S} protocol to transform the accumulated result back to secret sharing scheme. In total, it takes $2M$ \textit{Encryption}s, $2MN$ \textit{Addition}s, and $2KN$ \textit{Decryption}s under homomorphic encryption scheme. And the two transformation protocols need to communicate $(2M+2NK)$ ciphertexts, which is much longer than secret shares.
\end{itemize}

We will experimentally compare CRP-XGB and HEP-XGB and describe how to choose a proper one in Section \ref{secexp}.






\subsection{Secure XGB Prediction Algorithm}
We present a novel secure XGB prediction algorithm with the example in Figure \ref{figpred}. The upper part
displays the normal prediction process over a single tree. Prediction starts from
the root node and recursively chooses a child node determined by the split information.
Moving along the prediction path (shown in red arrows) until the leaf ($n_{1}\rightarrow n_{2}\rightarrow n_{5}$),
the corresponding weight ($w_{5}$) is finally returned
as the prediction. To facilitate the secure version, we introduce an one-hot indicator vector $S$ to mark the selected leaf node. The prediction could be regarded as
the inner product of S and W (a vector consists of all leaf weights).

\begin{figure}[htbp]
		\centering
		\includegraphics[width=0.43\textwidth]{pics/pred.pdf}
		\vskip -0.05in
		\caption{Illustration of secure tree prediction}\label{figpred}
% 		\vskip -0.15in
\end{figure}

Supposing that the intermediate nodes $n_{1}$ \& $n_{3}$ are split by
party A and $n_{2}$ is a dummy node for party A. On the contrary, party B is
only aware of the split information of $n_{2}$. Leaf weights are variables under
SS domain, each party holds one of the shares. The output model of our secure
training algorithm is distributed just as we marked in the bottom part of
Figure \ref{figpred}. 
It explains an innovative way to achieve
similar prediction process under the SS domain. Both parties first
generate leaf indicator vector locally. 
For each party (e.g., A), if its intermediate node has split
information (e.g. $n_{1}$ of party A), the unselected branch is abandoned (e.g. $n_{3}$ of party A). 
Otherwise, prediction continues on both branches (e.g. $n_{2}$ of party A).
The local indicator vector marks all the candidate leaves with the partial model.
Obviously, the intersection of local indicator vectors is equivalent to the
one-hot indicator vector $S$. So we transform the local indicator vector to
SS domain and get $S$ with an element-wise multiplication. The prediction
now can be computed efficiently with the weight vector and the indicator vector under SS domain.
By cumulating predictions of all the trees, we obtain the final prediction of XGB. %And additional sigmoid computation is necessary for classification tasks.

% \section{The proposed model: Secure XGB}\label{secxgb}
% In this section, we first elaborate the secure XGB training algorithm with the pseudocodes. % and extend the general XGB all the way to a secure HESS-XGB. 
% With the primitives in Section \ref{secprimitive}, we implement two versions, one is based on SS only and the other utilizes both HE and SS. % mechanism for further optimization.
% We finally present the secure prediction algorithm and implementation notes. 

% \subsection{Transformation Primitives}
% As the fundamental components
% of secure XGB, we first demonstrate the transformation primitives between \textit{HE}
% and \textit{SS}.

% \label{sectrans}
% %\begin{itemize}
% 	%\item 
	
% 	\textbf{H2S}: Transform a \textcolor[rgb]{0,0.6875,0.9375}{\textit{HE}} variable into a \textcolor[rgb]{0,0.6875,0.3125}{\textit{SS}} variable . The primitive is illustrated in Figure \ref{figh2s} and denoted as:
% 	\begin{equation}
% 	\textit{H2S}: (SK_{A} \text{\ \textbrokenbar\ } PK_{A}, \textcolor[rgb]{0,0.6875,0.9375}{\textit{$[x]_{A}$}} )\mapsto\left( \textcolor[rgb]{0,0.6875,0.3125}{\textit{$\left\langle x\right\rangle _{A}$}}\text{\ \textbrokenbar\ } \textcolor[rgb]{0,0.6875,0.3125}{\textit{$\left\langle x\right\rangle _{B}$}}\right). 
% 	%\label{formula7}
% 	\end{equation}
	
% 	\begin{figure}[t]
% 		\centering
% 		\includegraphics[width=0.5\textwidth]{pics/h2s.pdf}
% %		\vskip -0.15in
% 		\caption{H2S primitive}\label{figh2s}
% %		\vskip -0.05in
% 	\end{figure}
	
% 	The original variable $x$ can be a private data or an intermediate value. On the one hand,
% 	$x$ is encrypted by $PK_{A}$ and party B cannot decrypt the ciphertext. On the other hand, 
% 	Party A only gets ciphertext of the random share. Both parties have no access to the
% 	original variable, thus it is transformed securely with the help of \textit{HADD}.
% 	Symmetrically, for $[x]_{B}$, we have:
% 	\begin{equation}
% 	\textit{H2S}: (PK_{B}, \textcolor[rgb]{0,0.6875,0.9375}{\textit{$[x]_{B}$}} \text{\ \textbrokenbar\ }SK_{B})\mapsto\left( \textcolor[rgb]{0,0.6875,0.3125}{\textit{$\left\langle x\right\rangle _{A}$}}\text{\ \textbrokenbar\ } \textcolor[rgb]{0,0.6875,0.3125}{\textit{$\left\langle x\right\rangle _{B}$}}\right). 
% 	\end{equation}
% 	We denote the transformation as $\left\langle x\right\rangle=H2S([x]_{A})$ or $\left\langle x\right\rangle=H2S([x]_{B})$ for simplicity.
	
% 	%\item 
	
% 	\textbf{S2H}: Transform a \textcolor[rgb]{0,0.6875,0.3125}{\textit{SS}} variable into a \textcolor[rgb]{0,0.6875,0.9375}{\textit{HE}} variable . It is illustrated in  Figure \ref{figs2h} and denoted as:
% 	\begin{equation}
% 	\textit{S2H}: (PK_{A}, \textcolor[rgb]{0,0.6875,0.3125}{\textit{$\left\langle x\right\rangle _{A}$}} \text{\ \textbrokenbar\ } PK_{A}, \textcolor[rgb]{0,0.6875,0.3125}{\textit{$\left\langle x\right\rangle _{B}$}} )\mapsto\left( 
% 	\text{\ \textbrokenbar\ }  \textcolor[rgb]{0,0.6875,0.9375}{\textit{$[x]_{A}$}} \right). 
% 	%\label{formula7}
% 	\end{equation}
% 	\begin{figure}[t]
% 		\centering
% 		\includegraphics[width=0.5\textwidth]{pics/s2h.pdf}
% %		\vskip -0.15in
% 		\caption{S2H primitive}\label{figs2h}
% %		\vskip -0.05in
% 	\end{figure}
% 	In this case, Party A acts as encrypter and provides the public key. Party B receives the encrypted complementary share
% 	and computes the sum to get the related cipertext. Further computations could be executed by Party B in the \textit{HE} domain.
% 	Because Party B has no access to $SK_{A}$, the sum value is secure. \textit{HADD} is applied as a base primitive in
% 	this transformation as well. Similarly, we have:
% 	\begin{equation}
% 	\textit{S2H}: (PK_{B}, \textcolor[rgb]{0,0.6875,0.3125}{\textit{$\left\langle x\right\rangle _{A}$}} \text{\ \textbrokenbar\ } PK_{B}, \textcolor[rgb]{0,0.6875,0.3125}{\textit{$\left\langle x\right\rangle _{B}$}} )\mapsto\left( 
% 	  \textcolor[rgb]{0,0.6875,0.9375}{\textit{$[x]_{B}$}} \text{\ \textbrokenbar\ } \right). 
% 	%\label{formula7}
% 	\end{equation}
% 	We denote the transformation as $[x]_{A}=S2H(\left\langle x\right\rangle)$ or $[x]_{B}=S2H(\left\langle x\right\rangle)$ for simplicity.
% %\end{itemize}

% % \nosection{Theorem 1}
% % \textit{
% % Assume that the additively homomorphic cryptosystem is indistinguishable under chosen-plaintext attacks. Then, \textbf{H2S} and \textbf{S2H} are secure in semi-honest models.
% % }

% % \nosection{Proof}
% % The correctness and security of Theorem 1 can be easily proved following the simulation proof technique in \cite{lindell2017simulate}. 
% We now prove the transformation primitives are secure under the \emph{standard semi-honest model}, where a probabilistic polynomial-time adversary with semi-honest behaviors is considered. During the protocol execution with the honest party, the adversary will follow the protocol specification, but may attempt to obtain additional information about the honest party's input by analyzing the corrupted party's \emph{view}, \ie the transcripts it receives during the protocol execution. In order to ensure correctness and privacy, the following formal security definition is proposed \cite{goldreich2009foundations}. 

% \begin{definition}[Security in semi-honest model]
	
% Let $f = (f_1, f_2)$ be a \emph{deterministic} functionality and $\pi$ be a two-party protocol for computing $f$. Given the security parameter $\kappa$, and a pair of inputs $(x,y)$ (where $x$ is from $P_1$ and $y$ is from $P_2$), the view of $P_i$ ($i=1,2$) in the protocol $\pi$ is denoted as $\mathsf{view}^\pi_i(x, y, \kappa) = (w, r_i, m_i^1,\cdots, m_i^t)$, where $w\in\{x, y\}$, $r_i$ is the randomness used by $P_i$, and $m_i^j$ is the $j$-th message received by $P_i$; the output of $P_i$ is denoted as $\mathsf{output}_i^\pi(x, y, \kappa)$, 
% making up the joint output $\mathsf{output}^\pi(x, y, \kappa)$.
% We say that $\pi$ securely computes $f$ in semi-honest model if 
% \begin{itemize}
% 	\item There exist probabilistic polynomial-time simulators $\mathcal{S}_1$ and $\mathcal{S}_2$, such that
% $$\{\mathcal{S}_1(1^\kappa,x,f_1(x,y))\}_{x,y,\kappa}\cong\{\mathsf{view}_1^\pi(x,y,\kappa)\}_{x,y,\kappa},$$
% $$\{\mathcal{S}_2(1^\kappa,y,f_2(x,y))\}_{x,y,\kappa}\cong\{\mathsf{view}_2^\pi(x,y,\kappa)\}_{x,y,\kappa}.$$
% 	\item The joint output and the functionality output satisfy
% 	$$\{\mathsf{output}^\pi(x, y, \kappa)\}_{x,y,\kappa}\cong\{f(x,y)\}_{x,y,\kappa},$$
% \end{itemize}
% where $x, y\in \{0, 1\}^*$, and $\cong$ denotes computationally indistinguishablity.
% \end{definition}


% \begin{theorem}
% 	Assume that the additively homomorphic cryptosystem $\Pi=(\textsf{KeyGen}$, $ \textsf{Enc}$, $\textsf{Dec})$ is indistinguishable under chosen-plaintext attacks. Then, \textbf{H2S Protocol} (denoted as $\pi_1$) is secure in semi-honest model.
% \end{theorem}
% \begin{proof}
%     By following the steps in figure \ref{figh2s}, the correctness is obliviously obtained from the additive homomorphism definition.  We now prove that we can construct two simulators $\mathcal{S}_{\mathcal{A}}$ and $\mathcal{S}_{\mathcal{B}}$, such that
%     \begin{small}
% 	\begin{eqnarray}
% 		\{\mathcal{S}_{\mathcal{A}}(1^\kappa,SK_A,\langle x\rangle_A)\}_{SK_A,[x]_A,\kappa}\cong\{\mathsf{view}_{\mathcal{A}}^{\pi_1}(SK_A,[x]_A,\kappa)\}_{SK_A,[x]_A,\kappa},\label{eqn1}\\
% 		\{\mathcal{S}_{\mathcal{B}}(1^\kappa,[x]_A,\langle x\rangle_B)\}_{SK_A,[x]_A,\kappa}\cong\{\mathsf{view}_{\mathcal{B}}^{\pi_1}(SK_A,[x]_A,\kappa)\}_{SK_A,[x]_A,\kappa}, \label{eqn2}
% 	\end{eqnarray}
% 	\end{small}

% 	where $\mathsf{view}_{\mathcal{A}}^{\pi_1}$ and $\mathsf{view}_{\mathcal{B}}^{\pi_1}$ denote the views of $\mathcal{A}$ and $\mathcal{B}$, respectively.We prove the above equations for a corrupted $\mathcal{A}$ and a corrupted $\mathcal{B}$, respectively.
	
% 	\paragraph{Corrupted $\mathcal{A}$} In this case, we construct a probabilistic polynomial-time simulator $\mathcal{S}_{\mathcal{A}}$ that, when given the security parameter $\kappa$, $\mathcal{A}$'s input $SK_A$ and output $\langle x \rangle_A$, can simulate the view of $\mathcal{A}$ in the protocol execution. 
% 	%To this end, we first analyze $\mathcal{A}$'s view $\mathsf{view}_{\mathcal{A}}^{\pi_1}(SK_A,[x]_A,\kappa)$ in \textbf{H2S Protocol}. 
% 	In \textbf{H2S Protocol}, the only message obtained by $\mathcal{A}$ is the ciphertext $[\langle x\rangle_A]_A$. Therefore, $\mathsf{view}_{\mathcal{A}}^{\pi_1}(SK_A,[x]_A,\kappa)$ consists of $\mathcal{A}$'s input $SK_A$, the randomness $r_{\mathcal{A}}$, and the ciphertext $[\langle x\rangle_A]_A$.
	
% 	Given $\kappa$, $SK_A$, and $\langle x\rangle_A$, $\mathcal{S}_{\mathcal{A}}$ simulates
% 	$\mathsf{view}_{\mathcal{A}}^{\pi_1}(SK_A,[x]_A,\kappa)$ by encrypting $\langle x\rangle_A$ with $\mathcal{A}$'s public key $PK_A$, and obtains $[\langle x\rangle_A]'_A$. Therefore, we have the following two equations:
	
% 	$$\mathsf{view}_{\mathcal{A}}^{\pi_1}(SK_A,[x]_A,\kappa))=(SK_A, r_{\mathcal{A}}, [\langle x\rangle_A]_A),$$
% 	$$\mathcal{S}_{\mathcal{A}}(1^\kappa,SK_A, \langle x\rangle_A)=(SK_A,r_{\mathcal{A}},[\langle x\rangle_A]'_A).$$
	
% 	We note that as the additively homomorphic cryptosystem $\Pi$ is indistinguishable under chosen-plaintext attacks, the probability distributions of $\mathcal{A}$'s view and $\mathcal{S}_{\mathcal{A}}$'s output are computationally indistinguishable.
% 	We thereby claim that Equation (\ref{eqn1}) holds.
	
% 	\paragraph{Corrupted $\mathcal{B}$} In this case, we construct a probabilistic polynomial-time simulator $\mathcal{S}_{\mathcal{B}}$, when given the security parameter $\kappa$, $\mathcal{B}$'s input $[x]_A$ and output $\langle x\rangle_B$, can simulate the view of $\mathcal{B}$ in the protocol execution. In \textbf{H2S Protocol}, $\mathcal{B}$ does not receive any messages from $\mathcal{A}$. Therefore, $\mathsf{view}_{\mathcal{B}}^{\pi_1}(SK_A,[x]_A,\kappa)$ consists of $\mathcal{B}$'s input $[x]_A$ and the randomness $r_{\mathcal{B}}$.
%      $\mathcal{S}_{\mathcal{B}}$ generates a simulation by directly outputting $([x]_A,r_{\mathcal{B}})$. Therefore, we have the following two equations:
	
% 	$$\mathsf{view}_{\mathcal{B}}^{\pi_1}(SK_A,[x]_A,\kappa)=([x]_A,r_{\mathcal{B}}),$$
% 	$$\mathcal{S}_{\mathcal{B}}(1^\kappa, [x]_A,\langle x\rangle_B)=([x]_A,r_{\mathcal{B}}).$$
	
	
% 	We note that the probability distributions of $\mathcal{B}$'s view and $\mathcal{S}_{\mathcal{B}}$'s output are identical.
% 	We thereby claim that Equation (\ref{eqn1}) holds.

	
% 	In summary, \textbf{H2S Protocol} is secure in semi-honest model.
% \end{proof}

% \begin{theorem}
% 	Assume that the additively homomorphic cryptosystem $\Pi=(\textsf{KeyGen}$, $ \textsf{Enc}$, $\textsf{Dec})$ is indistinguishable under chosen-plaintext attacks. Then, \textbf{S2H Protocol} (denoted as $\pi_2$) is secure in semi-honest model.
% \end{theorem}


% \begin{proof}
% 	We neglect the simple correctness analysis and prove that we can construct two simulators $\mathcal{S}_{\mathcal{A}}$ and $\mathcal{S}_{\mathcal{B}}$, such that
% 	\begin{small}
% 	\begin{eqnarray}
% 		\{\mathcal{S}_{\mathcal{A}}(1^\kappa,\langle x \rangle_A)\}_{\langle x\rangle_A,\langle x\rangle_B,\kappa}\cong\{\mathsf{view}_{\mathcal{A}}^{\pi_2}(\langle x\rangle_A,\langle x\rangle_B,\kappa)\}_{\langle x\rangle_A,\langle x\rangle_B,\kappa},\label{eqn3}\\
% 		\{\mathcal{S}_{\mathcal{B}}(1^\kappa,\langle x\rangle_B,[x]_A)\}_{\langle x\rangle_A,\langle x\rangle_B,\kappa}\cong\{\mathsf{view}_{\mathcal{B}}^{\pi_2}(\langle x\rangle_A,\langle x\rangle_B,\kappa)\}_{\langle x\rangle_A,\langle x\rangle_B,\kappa}, \label{eqn4}
% 	\end{eqnarray}
% 	\end{small}
% 	%where $\mathsf{view}_{\mathcal{A}}^{\pi_2}$ and $\mathsf{view}_{\mathcal{B}}^{\pi_2}$ denote the views of $\mathcal{A}$ and $\mathcal{B}$, respectively.
	
% 	%We prove the above equations for a corrupted $\mathcal{A}$ and a corrupted $\mathcal{B}$, respectively.
% 	\paragraph{Corrupted $\mathcal{A}$} In \textbf{S2H Protocol}, $\mathcal{A}$ does not receive any messages from $\mathcal{B}$. Therefore, $\mathsf{view}_{\mathcal{A}}^{\pi_2}(\langle x\rangle_A,\langle x\rangle_B,\kappa)$ consists of $\mathcal{A}$'s input $\langle x \rangle_A$ and the randomness $r_{\mathcal{A}}$.
	

	
% 	Given $\kappa$ and $\langle x \rangle_A$, $\mathcal{S}_{\mathcal{A}}$ generates a simulation by directly outputting $(\langle x \rangle_A, r_{\mathcal{A}})$. Therefore, we have the following two equations:
	
% 	$$\mathsf{view}_{\mathcal{A}}^{\pi_2}(\langle x\rangle_A,\langle x\rangle_B,\kappa)=(\langle x \rangle_A,r_{\mathcal{A}}),$$
% 	$$\mathcal{S}_{\mathcal{A}}(1^\kappa,\langle x \rangle_A)=(\langle x \rangle_A,r_{\mathcal{A}}).$$
	
% 	We note that the probability distributions of $\mathcal{A}$'s view and $\mathcal{S}_{\mathcal{A}}$'s output are identical.
% 	We thereby claim that Equation (\ref{eqn3}) holds.
	
	
% 	\paragraph{Corrupted $\mathcal{B}$} In \textbf{S2H Protocol}, the only message obtained by $\mathcal{B}$ is the ciphertext $[\langle x\rangle_A]_A$. Therefore, $\mathsf{view}_{\mathcal{B}}^{\pi_2}(\langle x\rangle_A,\langle x\rangle_B,\kappa)$ consists of $\mathcal{B}$'s input $\langle x \rangle_B$, the randomness $r_{\mathcal{B}}$, and the ciphertext $[\langle x\rangle_A]_A$.
	
% 	Given $\kappa$, $\langle x\rangle_B$, and $[x]_A$, $\mathcal{S}_{\mathcal{B}}$ generates a simulation as follows. It encrypts $\langle x\rangle_B$ with $\mathcal{A}$'s public key $PK_A$, and computes $[x]_A-[\langle x\rangle_B]_A$. Denote the computation result as $[\langle x\rangle_A]'_A$.\footnote{Actually here $\mathcal{S}_{\mathcal{B}}$ can just select a random plaintext, encrypts it, and takes the ciphertext as a simulation of $[\langle x\rangle_A]_A$.} Then, it generates $(\langle x \rangle_B,r_{\mathcal{B}},[\langle x\rangle_A]'_A)$ as the output. Therefore, we have the following two equations:
	
% 	$$\mathsf{view}_{\mathcal{B}}^{\pi_2}(\langle x\rangle_A,\langle x\rangle_B,\kappa)=(\langle x \rangle_B,r_{\mathcal{B}},[\langle x\rangle_A]_A),$$
% 	$$\mathcal{S}_{\mathcal{B}}(1^\kappa,\langle x \rangle_B,[x]_A)=(\langle x \rangle_B,r_{\mathcal{B}},[\langle x\rangle_A]'_A).$$
	
% 	We note that as the additively homomorphic cryptosystem $\Pi$ is indistinguishable under chosen-plaintext attacks, the probability distributions of $\mathcal{B}$'s view and $\mathcal{S}_{\mathcal{B}}$'s output are computationally indistinguishable.
% 	We thereby claim that Equation (\ref{eqn4}) holds.
	
	
% 	In summary, \textbf{S2H Protocol} is secure in semi-honest model.

	
% \end{proof}

% \subsection{Secure XGB Training Algorithm}
% We start from the general XGB training in Algorithm \ref{alg:trainxgb}. The inputs are a feature matrix $X$ (with $M$ samples and $N$ features) and the label vector $Y$. As an additive model, it first makes an initial guess (line 3), followed by the predictions from the $T$ tree models as revisions (line 8-20), where $T$ is the tree number of XGB. The colon equal ($:=$) represents a loop assignment. For example, line 7 assigns the base score to every element of the prediction vector as the initial prediction. 
% XGB simplifies the objective function with second-order approximation. The derivatives are updated during each iteration (line 11-12) with the previous predictions (line 16\&19). By iteratively calling the \textit{\textbf{BuildTree}} and \textit{\textbf{PredictTree}} functions, the tree models are constructed to minimize the given loss function. Finally, a model $F$ is returned with a base score and $T$ trees.
% % \begin{algorithm}[t] 
% % 	\begin{algorithmic}[1]  
% % 		\caption{Secure Training Algorithm of XGB}
% % 		\label{alg:trainxgb}  
% % 		\Function {TrainXGB}{$ X, Y, T$}
% % 		\State // \textit{Input} - $ X\colon\{ x\}_{M\times N} ^{i,j},  Y\colon\{ y\}_{M} ^{i}$
% % 		\State $f_{0}=ComputeBaseScore(Y)$
% % 		\State // Init tree model list
% % 		\State $F=[f_{0}]$
% % 		\State // Init prediction vector $\hat{Y}\colon\{ \hat{y}\}_{M} ^{i}$
% % 		\State $ \{ \hat{y}\} ^{i}\colon=f_{0}$
% % 		\For{$t=1,2,...,T$}
% % 		\State // Compute current first\&second order derivatives
% % 		\State // $G_{t-1}\colon\{ g_{t-1}\}_{M} ^{i}, H_{t-1}\colon\{ h_{t-1}\}_{M} ^{i}$
% % 		\State $G_{t-1}=ComputeGradient(Y, \hat{Y})$
% % 		\State $H_{t-1}=ComputeHessian(Y, \hat{Y})$
% % 		\State // Build a tree based on the derivatives and features
% % 		\State $f_{t}=\textit{\textbf{BuildTree}}(G_{t-1},H_{t-1}, X)$
% % 		\State // Compute prediction of current tree $\hat{Y}_{t}\colon\{ \hat{y}_{t}\}_{M}^{i}$
% % 		\State $\hat{Y}_{t}=\textit{\textbf{PredictTree}}(f_{t}, X)$
% % 		\State // Update the model list and prediction vector
% % 		\State $F.append(f_{t})$
% % 		\State $\{ \hat{y}\} ^{i}\colon=\{ \hat{y}\} ^{i}+\{ \hat{y}_{t}\} ^{i}$
% % 		\EndFor 
% % 		\State \Return $F$
% % 		\EndFunction
% % 	\end{algorithmic}  
% % \end{algorithm}


% \subsection{Secure \textit{BuildTree} and \textit{PredictTree}}
% The calculations of initial guess, first-order derivatives, and second-order derivatives depend on the specific
% loss function and can be computed with the secure computation primitives. So we focus on the key part of the
% framework, that is the \textit{\textbf{BuildTree}} and \textit{\textbf{PredictTree}}, as will be described in Algorithm \ref{alg:ssbuild}.%,\ref{alg:sssplit},\ref{alg:ssbuck}.

% \begin{algorithm}[htb] 
% 	\begin{algorithmic}[1]  
% 		\caption{Secure $BuildTree$ and $PredictTree$}
% 		\label{alg:ssbuild}  
% 		\Function {BuildAndPredict}{$G, H, X$}
% 		\State // \textit{Input} - $ G\colon\{ g\}_{M} ^{i}, H\colon\{ h\}_{M} ^{i}, X\colon\{ x\}_{M\times N} ^{i,j}$
% 		\State // Init root node
% 		\State $root=Node()$
% 		\State // Init sample indicator vector for root node $S\colon\{ s\}_{M} ^{i}$
% 		\State $\{ s\} ^{i}\colon=1$
% 		\State // Init candidate split matrix $V\colon \{ v\}_{N\times K} ^{j,k}$
% 		\State // Get shared $\langle G\rangle\colon\{ \langle g\rangle \}_{M}^{i}, \langle H\rangle\colon\{ \langle h\rangle \}_{M}^{i}, \langle S\rangle\colon\{ \langle s\rangle \}_{M}^{i}$
% 		\State $\{ \langle g\rangle \}^{i}\colon=N2S(\{ g\} ^{i})$
% 		\State $\{ \langle h\rangle \}^{i}\colon=N2S(\{ h\} ^{i})$
% 		\State $\{ \langle s\rangle \}^{i}\colon=N2S(\{ s\} ^{i})$
% 		\State // Split nodes from the root
% 		\State $\langle \hat{Y}\rangle=\textit{\textbf{SSSplitNode}}(root,\langle G\rangle, \langle H\rangle, \langle S\rangle, X, V )$
		
% 		\State \Return $root,\langle \hat{Y}\rangle$
% 		\EndFunction
% 	\end{algorithmic}
% \end{algorithm}
% %\vspace{-0.1in}

% Algorithm \ref{alg:ssbuild} mainly initializes the computation by transforming the necessary varibles, i.e.
% first-order derivative vector ($G$) and  second-order derivative vector ($H$) for all the samples, to the SS domain (line 9-10).
% For all the nodes in a tree, in order to record which samples belong to them, we introduce an indicator vector $S$ for each node. 
% For a certain node, if the $i$-th sample falls
% into it, we set $\{ s\} ^{i}$ to 1, otherwise to 0.
% Naturally, for the root node, all the samples belong to it, therefore, we initialize all the elements of its indicator vector to 1 (line 5-6). 
% To further preserve privacy, we transform the indicator vector to SS variable (line 11).
% In this way, the sum of the derivatives of the samples in a single node can be computed as the inner product of the indicator
% vector and the derivative vector, which can be securely computed by \textbf{SADD} \& \textbf{SMUL} primitives.

% For better illustration, we set up a split matrix $V$ (line 7), where $K$ is the bucket number for the candidate splits. The split matrix has two usages:
% (\romannumeral1) $\{ x\}^{i,j}\in \{ v\}^{j,k}.range$ means that the feature value of the $i$-th sample falls into
% the $k$-th bucket of the feature $j$; (\romannumeral2) $\{ x\} ^{i,j}\leq\{ v\} ^{j,k}.value$ means that the $i$-th sample belongs
% to left branch split by the $k$-th candidate split value of feature $j$. Because the feature matrix is vertically partitioned, the
% feature splits and bucket ranges could be precomputed locally without interactions. For computation efficiency concern, 
% we adopt the global proposal method in XGB \cite{chen2016xgboost} for split candidates. 

% After initialization, \textit{\textbf{SSSplitNode}} is
% called to split the tree top down from the root node to leaf nodes (line 13). In the process, the split information is recorded in the $Node$
% data structure and the prediction of current tree $\langle \hat{Y}\rangle$ is finally returned (line 14).



% Algorithm \ref{alg:sssplit} describes how to split a node in SS domain. Firstly, a termination check determines whether a node
% should split (line 4). 
% %The frequently-used prune conditions either need to reveal some intermediate result or leak the distribution information of samples. So we only terminate at the desired tree depth and the model is consisted of a batch of full binary trees. 
% When no further split is needed, the node is marked as a leaf node (line 5). 
% The leaf weight is securely computed with the SS variables (line 6), where
% $\lambda$ is the L2 regularization term described in Eq. \eqref{eqobj}. % on the weights, a common parameter for XGB algorithm. 
% The secretly shared predictions on
% current node are then computed by a element-wise secure multiplication (line 8). Note that, the leaf weight will only be assigned
% to the samples in this node and the predictions are set to 0 otherwise (with the original value $\{s\} ^{i}$ equals to 0).

% Next, with the node continue splitting, we enumerate all the split candidates and choose the best one with the highest gain (line 17-26).
% Before that, we compute the current node gain (line 11-13) and prepare the $g\&h$ cumulations in all the feature buckets (line 14-16). 
% \textit{\textbf{SSSumBucket}} is in charge of aggregating the $g\&h$ in each bucket, which will be presented in Section \ref{sec:work:hess:bucket}. 
% The best split information can be computed securely by using \textbf{SARGMAX} primitive (line 26), which outputs the index of feature bucket with the best gain.

% \begin{algorithm}%[H] 
% 	\begin{algorithmic}[1]  
% 		\caption{Secure $SplitNode$ based on SS}
% 		\label{alg:sssplit}  
% 		\Function {SSSplitNode}{$node,\langle G\rangle, \langle H\rangle, \langle S\rangle, X, V$}
% 		\State // \textit{Input} - $  \langle G\rangle\colon\{ \langle g\rangle\}_{M} ^{i}
% 		, \langle H\rangle\colon\{ \langle h\rangle\}_{M} ^{i}
% 		, \langle S\rangle\colon\{ \langle s\rangle\}_{M} ^{i}$
% 		\State //$\quad\quad and\ X\colon\{ x\}_{M\times N} ^{i,j}
% 		, V\colon \{ v\}_{N\times K} ^{j,k}$
% 		\If  {$terminate$}  
% 		\State $node.isLeaf=True$
% 		\State $node.\langle weight\rangle=\frac{\sum_{i}\{ \langle s\rangle\} ^{i}\cdot\{ \langle g\rangle\} ^{i}}{\sum_{i}\{ \langle s\rangle\} ^{i}\cdot\{ \langle h\rangle\} ^{i}+\langle\lambda\rangle}$
% 		\State // Compute prediction vector on leaf $\langle \hat{Y}\rangle\colon\{ \langle  y\rangle\}_{M}^{i}$
% 		\State $\{ \langle  y\rangle\}^{i}\colon=\{ \langle s\rangle\} ^{i}\cdot node.\langle weight\rangle$
% 		\State \Return $\langle \hat{Y}\rangle$
% 		\EndIf
% 		\State // Compute gain for current node
% 		\State$\langle sg\rangle=\sum_{i}\{  \langle g\rangle\} ^{i}, \quad\langle sh\rangle=\sum_{i}\{  \langle h\rangle\} ^{i}$ 
% 		\State $\langle  cgain\rangle=\frac{ \langle sg\rangle\cdot \langle sg\rangle}{\langle sh\rangle+\langle\lambda\rangle}$
% 		\State // Sum g\&h in the k-th bucket of feature j
% 		\State // $\langle BG\rangle\colon \{\langle bg\rangle\}_{M\times K}^{j,k},\quad\langle BH\rangle\colon\{\langle bh\rangle\}_{M\times K}^{j,k}$
% 		\State $\langle BG\rangle,\langle BH\rangle=\textit{\textbf{SumBucket}} (\langle G\rangle, \langle H\rangle, X, V)$
		
% 		\For{$j=1, 2, ...,N$}
% 		\State $\langle sg_{l}\rangle=N2S(0), \quad\langle sh_{l}\rangle=N2S(0)$
% 		\For{$k=1, 2, ... ,K$}
% 		\State $\langle sg_{l}\rangle=\langle sg_{l}\rangle+\{\langle bg\rangle\}^{j,k}, \langle sg_{r}\rangle=\langle sg\rangle-\langle sg_{l}\rangle$
% 		\State $\langle sh_{l}\rangle=\langle sh_{l}\rangle+\{\langle bh\rangle\}^{j,k}, \langle sh_{r}\rangle=\langle sh\rangle-\langle sh_{l}\rangle$
% 		\State // Compute gain matrix$\langle Gain\rangle\colon\{ \langle  gain\rangle\}_{N\times K}^{j,k}$
% 		\State $\{ \langle  gain\rangle\} ^{j,k}=\frac{ \langle sg_{l}\rangle\cdot \langle sg_{l}\rangle}{\langle sh_{l}\rangle+\langle\lambda\rangle}+\frac{ \langle sg_{r}\rangle\cdot \langle sg_{r}\rangle}{\langle sh_{r}\rangle+\langle\lambda\rangle}-\langle  cgain\rangle$
% 		\EndFor
% 		\EndFor
% 		\State $j_{best}, k_{best}=\arg\max\limits_{j,k}(\{ \langle  gain\rangle\} ^{j,k})$
% 		\State // Record split infomation at the party of feature $j_{best}$
% 		\State $node.splitFeat=j_{best}$
% 		\State $node.splitVal=\{ v\}^{j_{best},k_{best}}$
% 		\State // Init sample vectors for left child $S_{l}\colon\{ s_{l}\}_{M}^{i}$
% 		\State // and right child $S_{r}\colon\{ s_{r}\}_{M}^{i}$
% 		\If  {$\{ x\} ^{i,j}\leq\{ v\} ^{j_{best},k_{best}}.value$}  
% 		$\{ s_{l}\} ^{i}\colon=1$
% 		\Else \quad$\{ s_{l}\} ^{i}\colon=0$
% 		\EndIf
% 		\State $\{ s_{r}\} ^{i}\colon=1-\{ s_{l}\} ^{i}$
% 		\State // Get shared $\langle S_{l}\rangle\colon\{ \langle s_{l}\rangle\}_{M}^{i}
% 		, \langle S_{r}\rangle\colon\{ \langle s_{r}\rangle\}_{M}^{i}$
% 		\State $\{ \langle s_{l}\rangle\} ^{i}\colon=N2S(\{ s_{l}\} ^{i})
% 		,\ \{ \langle s_{l}\rangle\} ^{i}\colon=\{ \langle s_{l}\rangle\} ^{i}\cdot \{ \langle s\rangle\} ^{i}$
% 		\State $\{ \langle s_{r}\rangle\} ^{i}\colon=N2S(\{ s_{r}\} ^{i})
% 		,\ \{ \langle s_{r}\rangle\} ^{i}\colon=\{ \langle s_{r}\rangle\} ^{i}\cdot \{ \langle s\rangle\} ^{i}$
% 		\State // Get shared $\langle G_{l}\rangle\colon\{ \langle g_{l}\rangle\}_{M}^{i}
% 		, \langle H_{l}\rangle\colon\{ \langle h_{l}\rangle\}_{M}^{i}$
% 		\State $
% 		\{ \langle g_{l}\rangle\} ^{i}\colon=\{ \langle s_{l}\rangle\} ^{i}\cdot \{ \langle g\rangle\} ^{i}$
% 		\State $
% 		\{ \langle h_{l}\rangle\} ^{i}\colon=\{ \langle s_{l}\rangle\} ^{i}\cdot \{ \langle h\rangle\} ^{i}$
% 		\State // Get shared $\langle G_{r}\rangle\colon\{ \langle g_{r}\rangle\}_{M}^{i}
% 		, \langle H_{r}\rangle\colon\{ \langle h_{r}\rangle\}_{M}^{i}$
% 		\State $\{ \langle g_{r}\rangle\} ^{i}\colon=\{ \langle s_{r}\rangle\} ^{i}\cdot \{ \langle g\rangle\} ^{i}$
% 		\State $\{ \langle h_{r}\rangle\} ^{i}\colon=\{ \langle s_{r}\rangle\} ^{i}\cdot \{ \langle h\rangle\} ^{i}$
% 		\State // Init left child and right child
% 		\State $left=Node(), \quad right=Node()$
% 		\State // Prediction of left/right branch $\langle P_{l/r}\rangle\colon\{\langle p_{l/r}\rangle\}_{M}^{i}$
% 		\State $\langle P_{l}\rangle=SSSplitNode(left, \langle S_{l}\rangle, \langle G_{l}\rangle, \langle H_{l}\rangle, X, V)$
% 		\State $\langle P_{r}\rangle=SSSplitNode(right, \langle S_{r}\rangle, \langle G_{r}\rangle, \langle H_{r}\rangle, X, V)$
% 		\State // Combine prediction vectors as $\langle P\rangle\colon\{\langle p\rangle\}_{M}^{i}$
% 		\State $\{\langle p\rangle\}^{i}\colon=\{\langle p_{l}\rangle\}^{i}+\{\langle p_{r}\rangle\}^{i}$
% 		\State \Return $P$
% 		\EndFunction
% 	\end{algorithmic}  
% \end{algorithm}

% The split feature and split value pair are then reconstructed and recorded by the feature owner (line 27-29). 
% According to the split information, we then split the samples into left and right branches and generate related indicator vectors 
% for child nodes (line 30-44). Finally, we recursively call the \textit{\textbf{SSSplitNode}} function to split the child 
% nodes (line 46-49). Note that the element-wise summation of $\langle P_{l}\rangle$ \& $\langle P_{r}\rangle$ combines the predictions
% of both branches and outputs the belonging leaf weight for every sample (line 51). The security proof of Algorithm \ref{alg:sssplit} can be found in Appendix \ref{proof-splitnode}. 

% \begin{algorithm}[t] 
% 	\begin{algorithmic}[1]  
% 		\caption{Secure $SumBucket$ based on SS}
% 		\label{alg:ssbuck}  
% 		\Function {$SSSumBucket$}{$\langle G\rangle, \langle H\rangle, X, V$}
% 		\State // \textit{Input} - $  \langle G\rangle\colon\{ \langle g\rangle\}_{M} ^{i}
% 		, \langle H\rangle\colon\{ \langle h\rangle\}_{M} ^{i}$
% 		\State //$\quad\quad and\ X\colon\{ x\}_{M\times N} ^{i,j}
% 		, V\colon \{ v\}_{N\times K} ^{j,k}$
		
% 		\For{$j=1, 2, ...,N$}
% 		\For{$k=1, 2, ... ,K$}
% 		\If{$\{ x\}^{i,j}\in \{ v\}^{j,k}.range$}
% 		$\{ s_{jk}\} ^{i}\colon=1$
% 		\Else \quad$\{ s_{jk}\} ^{i}\colon=0$
% 		\EndIf
% 		\State $\{ \langle s_{jk}\rangle\} ^{i}\colon=N2S(\{ s_{jk}\} ^{i})$
% 		\State // Sum g\&h in bucket
% 		\State $\{\langle bg\rangle\}^{j,k}=\sum_{i}\{ \langle s_{jk}\rangle\} ^{i}\cdot\{  \langle g\rangle\} ^{i}$
% 		\State $\{\langle bh\rangle\}^{j,k}=\sum_{i}\{ \langle s_{jk}\rangle\} ^{i}\cdot\{  \langle h\rangle\} ^{i}$
% 		\EndFor
% 		\EndFor
% 		\State \Return $\{\langle bg\rangle\}^{j,k},\{\langle bh\rangle\}^{j,k}$
% 		\EndFunction
% 	\end{algorithmic}  
% \end{algorithm}

% \subsection{Secure Bucket Cumulator}\label{sec:work:hess:bucket}
% We propose two versions of secure bucket cumulator. 

% \nosection{SS Bucket Cumulator}
% We first present how to securely compute \textit{\textbf{SumBucket}} in SS domain only in 
% Algorithm \ref{alg:ssbuck}. %is the final piece of the jigsaw puzzle. 
% The indicator vector trick is employed
% again to record whether a sample falls into a specific bucket (line 6-7). $\{ s_{jk}\} ^{i}$ is set to 1
% if the $i$-th sample falls into the $k$-th bucket of feature $j$. $\{ s_{jk}\}_{M}$ is a column vector for the $k$-th bucket of feature $j$. 
% Then the bucket cumulation of $g\&h$ turns out to be the inner product of the indicator vector and the derivative vector (line 9-12).

% \nosection{HESS Bucket Cumulator}
% We then implement the \textit{\textbf{SumBucket}} based on HESS framework (in Algorithm \ref{alg:hessbuck}).
% %instead of the SS version. 
% The key insight is transforming the $g\&h$ into HE domain and cumulating them by the cipertexts. 
% Both parties first get the variables under HE domains (line 4-8). Each party initializes the indicator
% vector for current bucket (line 11-13) and cummulates the encrypted $g\&h$ (line 14-17). 
% %The indicator vector can be locally generated and used because the feature matrix is vertically partitioned. 
% The cumulation of a feature is maintained by the party who owns it.
% After the computation, the HE variables are transformed back to SS variables for further computations (line 18-20). 
% We can see from Algorithm \ref{alg:hessbuck} that, the encrypted $g\&h$ are shared among the nodes in the same tree, thus the ciphertexts only need to be communicated once. 
% %Moreover, because the cumulations are under the HE domain, the initial share and interaction communication cost of SS variable is avoided. 
% %Intuitively, the HESS version wins in terms of bandwidth, which is quite a practical progress.
% We will theoretically analyze the complexities of SS based SumBucket and HESS based SumBucket in Section \ref{seccomp}, and prove their security in Appendix \ref{proof-ss} and \ref{proof-hess}. 

% From now on, we name the secure XGB with SS SumBucket as \textbf{SS-XGB}, and term the secure XGB with HESS SumBucket as \textbf{HESS-XGB}. 

% \begin{algorithm}[htb] 
% 	\begin{algorithmic}[1]  
% 		\caption{Secure $SumBucket$ based on HESS}
% 		\label{alg:hessbuck}  
% 		\Function {$HESSSumBucket$}{$\langle G\rangle, \langle H\rangle, X, V$}
% 		\State // \textit{Input} - $  \langle G\rangle\colon\{ \langle g\rangle\}_{M} ^{i}
% 		, \langle H\rangle\colon\{ \langle h\rangle\}_{M} ^{i}$
% 		\State //$\quad\quad and\ X\colon\{ x\}_{M\times N} ^{i,j}
% 		, V\colon \{ v\}_{N\times K} ^{j,k}$
% 		\State // Transform SS variables to HE
% 		\State // $[ G]_{A}\colon\{ [ g]_{A}\}_{M} ^{i}
% 		,\ [ G]_{B}\colon\{ [ g]_{B}\}_{M} ^{i}$
% 		\State $\{ [ g]_{A}\}^{i}\colon=S2H(\{ \langle g\rangle\}^{i})
% 		,\{ [ g]_{B}\}^{i}\colon=S2H(\{ \langle g\rangle\}^{i}$
% 		\State // $[ H]_{A}\colon\{ [ h]_{A}\}_{M} ^{i}
% 		,\ [ H]_{B}\colon\{ [ h]_{B}\}_{M} ^{i}$
% 		\State $\{ [ h]_{A}\}^{i}\colon=S2H(\{ \langle h\rangle\}^{i})
% 		,\{ [ h]_{B}\}^{i}\colon=S2H(\{ \langle h\rangle\}^{i}$
% 		\For{$j=1, 2, ...,N$}
% 		\For{$k=1, 2, ... ,K$}
% 		\If{$\{ x\}^{i,j}\in \{ v\}^{j,k}.range$}
% 		$\{ s_{jk}\} ^{i}=1$
% 		\Else \quad$\{ s_{jk}\} ^{i}=0$
% 		\EndIf
% 		\State // Suppose feature j is at one party $P\in \{A,B\}$
% 		\State // Sum g\&h encrypted by the other party $\bar{P}$
% 		\State $\{[ bg]_{\bar{P}}\}^{j,k}=\sum_{i}\{  s_{jk}\} ^{i}\cdot\{  [ g]_{\bar{P}}\} ^{i}$
% 		\State $\{[ bh]_{\bar{P}}\}^{j,k}=\sum_{i}\{  s_{jk}\} ^{i}\cdot\{  [ h]_{\bar{P}}\} ^{i}$
% 		\State // Transform HE variables to SS
% 		\State $\{\langle bg\rangle\}^{j,k}=H2S(\{[ bg]_{\bar{P}}\}^{j,k})$
% 		\State $\{\langle bh\rangle\}^{j,k}=H2S(\{[ bh]_{\bar{P}}\}^{j,k})$
% 		\EndFor
% 		\EndFor
% 		\State \Return $\{\langle bg\rangle\}^{j,k},\{\langle bh\rangle\}^{j,k}$
% 		\EndFunction
% 	\end{algorithmic}  
% \end{algorithm}

% \subsection{Secure XGB Prediction Algorithm}
% We then present a novel secure XGB prediction algorithm with the example in Figure \ref{figpred}. The upper part
% displays the normal prediction process over a single tree. Prediction starts from
% the root node and recursively chooses a child node determined by the split information.
% Moving along the prediction path (shown in red arrows) until the leaf ($n_{1}\rightarrow n_{2}\rightarrow n_{5}$),
% the corresponding weight ($w_{5}$) is finally returned
% as the prediction. To facilitate the secure version, we introduce an one-hot indicator vector $S$ to mark the selected leaf node. The prediction could be regarded as
% the inner product of S and W (a vector consists of all leaf weights).

% Supposing that the intermediate nodes $n_{1}$ \& $n_{3}$ are split by
% party A and $n_{2}$ is a dummy node for party A. On the contrary, party B is
% only aware of the split information of $n_{2}$. Leaf weights are variables under
% SS domain, each party holds one of the shares. The output model of our secure
% training algorithm is distributed just as we marked in the bottom part of
% Figure \ref{figpred}. 
% It explains an innovative way to achieve
% similar prediction process under the SS domain. Both parties first
% generate leaf indicator vector locally. 
% For each party (e.g., A), if its intermediate node has split
% information (e.g. $n_{1}$ of party A), the unselected branch is abandoned (e.g. $n_{3}$ of party A). 
% Otherwise, prediction continues on both branches (e.g. $n_{2}$ of party A).
% The local indicator vector marks all the candidate leaves with the partial model.
% Obviously, the intersection of local indicator vectors is equivalent to the
% one-hot indicator vector $S$. So we transform the local indicator vector to
% SS domain and get $S$ with an element-wise multiplication. The prediction
% now can be computed efficiently with the weight vector and the indicator vector under SS domain.
% By cumulating predictions of all the trees, we obtain the final prediction of XGB. %And additional sigmoid computation is necessary for classification tasks.

% \begin{figure}[t]
% 		\centering
% 		\includegraphics[width=0.43\textwidth]{pics/pred.pdf}
% %		\vskip -0.15in
% 		\caption{Illustration of secure tree prediction}\label{figpred}
% %		\vskip -0.1in
% \end{figure}

% \subsection{Implementation Details}
% \label{secimp}
% %Besides the general description of the algorithm, there are 
% We now describe 
% several implementation essentials in details.

% \nosection{Algorithm parameters} Our implementation supports most parameters of XGB, e.g. the number of estimators, the max depth of a tree, the learning rate, and L2 regularization. 
% Besides, we also support sampling and pruning. 
% In practice, \textit{sampling} is an important strategy to prevent overfitting and increase the tree diversity, %, which contribute much to the accuracy.
% which includes feature (column) sampling and sample (row) sampling. 
% First, for column sampling, when fitting trees, both parties locally permute the feature indexes and select features according to the preset sampling rate.
% After it, the following computations are based on the permuted indexes instead of the original ones. 
% %Feature sampling by tree is easy to support in Algorithm \ref{alg:ssbuild}. Before fitting a tree, the parties locally permute the feature indexes and select the feature according to the sampling rate parameter.
% %The following computation is based on the permuted indexes and it additionally avoid the information leakage in Algorithm \ref{alg:sssplit}. 
% When recovering the bucket information (line 26 in Algorithm \ref{alg:sssplit}), the split feature index is permuted and the mapping relation is only available at the owner party, which avoid information leakage. 
% As for the row sampling, it first takes an extra round of communication for both parties to agree on the selected samples at the beginning of Algorithm \ref{alg:ssbuild}. 
% After it, row sampling can be done by initializing the selected samples to 1 for the root node (line 6). %, only these samples will take effect in the later computation. 
% \textit{Pruning} is another important strategy for XGB. 
% %is hard to support in MPC frameworks, because the gain value and weight sum are intermediate infomations that are not allowed to reveal.
% The best prune metric is split gain, which indicates whether a further partition is needed. 
% We simulate the pruning operation by introducing a dummy bucket and dividing all samples at left branch, which means that the left child is a copy of the parent node. 
% %Dummy computations will continue and repeat until reaching the leaf nodes, where the weight is computed. 
% In this way, we enjoy the benefit
% of pruning without revealing any intermediate values.

% % \textbf{Sample Alignment}: the joint parties need to align the samples by ID before running the algorithm. 
% % \textit{Private Set Intersection} is a well-known cryptographic technique that compute the elements in the
% % intersection and reveals nothing else. In terms of the bandwidth limit in our scenario, the variants based
% % on Diffie-Hellman key agreement are competitive choices. Specifically, the communication complexity is very small
% % implemented with the compact elliptic curve groups(ECDH-PSI)\cite{bernstein2006curve25519}. 

% \nosection{Fixed-point Arithmetic} Multi-party computation primitives only work in a finite field such as integers modulo $2^k$, which is computationally beneficial \cite{damgaard2012multiparty}.
% %such as the integers modulo a prime. Replacing the prime modulus with $2^k$ is a more popular setting currently, whichis computationally beneficial\cite{damgaard2012multiparty}. 
% To support decimal arithmetic, we adopt  truncate based fixed-point representation in \cite{mohassel2017secureml}. %The representation is easy to support and inherits the security of the integer arithmetic. But extra attention should be paid to the truncation operation after each multiplication. 
% %We follow the truncation method proposed in \cite{mohassel2017secureml} and truncate the product shares independently. 
% It has been proven that, with high probability, the reconstructed product is at most 1 bit off in the least significant position of the fractional part. This small truncation error is generally tolerable for machine learning applications
% with sufficient fractional bits. We use 20 out of 64 bits (i.e. $k=64$) to represent the fractional part in practice.

% \nosection{Additively Homomorphic Encryption} 
% %In the algorithm, only the homomorphic addition is in need, so partially homomorphic cryptosystems that support
% Additively homomorphic encryption are widely used in practice. 
% We implement two popular additively homomorphic encryption, i.e.,  Paillier \cite{paillier1999public} and Okamoto-Uchiyama (OU) \cite{okamoto1998new}.
% We will compare their performance in experiment. %and will employ the OU variant in \cite{coron1999accelerating}  and set the key size $l=2048$. 
% We can further speed up the encryption process by appropriate pre-computing. Specifically, we find that 
% about 95\% of the time is spending on the random generation and corresponding exponentiation, which is irrelevant to the plaintext
% and could be moved to the offline process. In terms of the transformation primitives mentioned in section \ref{sectrans}, there is another
% notable security concern. Because the plaintext space under the HE domain is $\mathbb{Z}_{2^{l}}$, instead of $\mathbb{Z}_{2^{k}}$, we have to set a security
% parameter $\sigma$ and pick the random number $r \in \mathbb{Z}_{2^{k+\sigma}}$. The probability of information leaking is then reduced
% to $2^{-\sigma}$, where we set $\sigma =40$. %Besides, there should be a modulo operation after the decryption.

% \nosection{Secret Sharing}
% Online speed-up is also enabled in the SS domain by generating the Beaver's triples offline. 
% Zero sharing technique further reduces the interaction cost with the help of pseudo-random functions (PRF) \cite{mohassel2018aby3}. 
% Moreover, sigmoid function is crucial for the classification problems. We approximate sigmoid function by Taylor expansion and reduce 
% it to \textbf{SADD} \& \textbf{SMUL} operations. As the basis of the \textbf{SARGMAX}, we need two more primitives. One primitive is used 
% to compare two shared values (\textbf{CMP}) and the other is multiplexers for conditional expressions (\textbf{MUX}).
% We make use of Boolean sharing in \cite{mohassel2017secureml} to implement the \textbf{CMP} primitive by judging
% the shared sign bit of the subtraction. A bunch of \textbf{MUX} operations take the pairwise comparison results and the related index shares as inputs
% and finally return the index for the max value. To accelerate the process, we can utilize binary tree reduction trick.

% \section{Complexity Analysis}\label{seccomp}
% In this section,  we take a close look at the bucket cumulation (\textit{SumBucket}) algorithms and give their theoretical complexity analysis. 
% %which reminds us of the optimation of the HESS framework.

% \subsection{Computation Complexity}\label{subseccomp}

% First, we analyze the computation complexity of SS based \textit{SumBucket} in Algorithm \ref{alg:ssbuck}. 
% To do this, we express it in a concise way with matrices. 
% First, the indicator vectors ($\{s_{jk}\}$) are generated by enumerating all the features and buckets. Second, the 
% horizontally concatenated vectors form an indicator matrix $S_{M\times NK}$, where $NK=N\times K$ is the
% total bucket number. We then transform $S_{M\times NK}$ to SS domain as $\langle S\rangle$. 
% Next, $\langle G\rangle_{M\times 1}$ and
% $\langle H\rangle_{M\times 1}$ are horizontally concatenated as well and transposed to a shared matrix $\langle R\rangle_{2\times M}$.
% The computation in line 11-12 becomes a shared matrix multiplicaiton $\langle C\rangle_{2\times NK}=\langle R\rangle \times \langle S\rangle$,
% where each row is the cumulation of $g$ or $h$ for all the buckets. Note that the indicator matrix $S$ is a large sparse 0/1 matrix,
% while $R$ is a relatively small dense matrix. Obviously, the size of matrix $S$ is exploded with the feature number. SS domain cannot handle the sparsity and the computation is as tedious as the dense matrices. 

% On the contrary, the HESS based \textit{SumBucket} in Algorithm \ref{alg:hessbuck} makes use of locally generated sparse $S$ directly.
% With the plaintext of $S$, only the necessary computations are executed. 
% However, it involves extra computation under HE domain. We introduce $t1, t2, t3$ to notate the average encryption time, homomorphic addition time, and
% decryption time respectively. It takes $2M\cdot t1$ to encrypt the matrix $R$ (line 6 \& 8). In line 16-17, there are two homomorphic
% additions for each element in feature matrix because $g$ \& $h$ are added to the corresponding bucket, i.e. $2MN\cdot t2$. When
% transforming the encrypted cumulations $\left[C\right]$ to the SS domain (line 19-20), $2NK\cdot t3$ is needed for decryption. Overall,
% the HESS version needs $T1 = 2M\cdot t1 + 2MN\cdot t2 + 2NK\cdot t3$ to cumulate.

% \subsection{Communication Complexity}
% The multiplication operation needs communications between two parties which becomes a bottleneck when it involves large matrices. 
% Also, sparse matrices are widely used in machine learning and
% the heavy communication traffic makes secure algorithms unrealistic. 
% In industry settings, bandwidth bottleneck is harder to break than computation bottleneck, especially for external collaborations. Even with the offline Beaver's Triple generation and Zero sharing, it still needs online communications 
% %to reveal the public differences 
% \cite{beaver1991efficient}. 
% For SS based \textit{SumBucket}, the communications are bidirectional and proportional to matrices
% $\langle R\rangle$ \& $\langle S\rangle$. 
% Suppose the variables are $l1$-bits, then, the total communication costs are $L_{SS}=2\cdot \left(MNK+2M\right)\cdot l1$ bits. 
% In constract, the HESS based \textit{SumBucket} only
% transfers the encrypted share matrix $\left[\langle R\rangle_{P}\right]_{P}$ to the opposite party $\bar{P}$  (for \textbf{S2H}) and receives
% the encrypted shares $\left[\langle C\rangle_{P}\right]_{P}$ (for \textbf{H2S}). 
% Assume the key size is $l2$-bits, then
% it spends $L_{HESS}=2\cdot \left(2M+2NK\right)\cdot l2$ bits. 

% We now study under what circumstances $L_{SS}$ will be greater than $L_{HESS}$. To do this, we let $L_{SS}/L_{HESS}>1$, then
% \begin{equation}
% \frac{2\cdot \left(MNK+2M\right)\cdot l1}{2\cdot \left(2M+2NK\right)\cdot l2}>1 \Rightarrow NK>\frac{2\cdot\frac{l2}{l1}\cdot M}{M-2\cdot\frac{l2}{l1}}.
% \end{equation}
% Following the setting in Section \ref{secimp}, $l1=64$ and $l2\approx 2300$ (average ciphertext length for 2048 bits key). We replace them in the above equation, since $M$ is the sample size which is much bigger than 72, and thus we get
% \begin{equation}
% NK>\frac{72M}{M-72}\xrightarrow{M\gg72}NK>72.
% \end{equation}
% In other words, the HESS version outperforms the SS one in terms of communication cost when the total bucket number $NK > 72$. 

% \subsection{Algorithm Choice}
% %The above complexity analysis serves as a guidance for practitioners to choose from the two training algorithm.
% % Given a dataset, with the values of $M$ (sample size), $N$ (feature size), and $K$ (average kucket number of all the features), one can easily choose the algorithm with the best communication cost. 
% %HESS framework makes a trade-off between the communication and the computation. In practice, the SS domain computations are negligible with respect to the costly homomorphic operations and the communication time of the HESS framework is much less than the SS mehthod.
% HESS-XGB saves the communication time by $T2=(L_{SS}-L_{HESS})/B$, where $B$ is the bandwidth limit in practice. But it also brings about additional homomorphic computation time $T1$(in section \ref{subseccomp}). By comparing $T1$ and $T2$, we can choose a more appropriate one from the two training algorithms.
% %we can choose a better framework for current settings and our HESS framework always brings out valuable promotions in privacy preserving machine learning.












==> proof.tex <==
\appendix
\section{Security Proof}\label{proof}
\subsection{SumBucket based on SS}\label{proof-ss}

% \begin{small}
% \begin{tcolorbox}[colback=white,arc=0pt,outer arc=0pt,boxrule=0.7pt,enhanced,breakable,fontupper=\linespread{.8}\selectfont]
% \textbf{Functionality of SumBucket based on SS $\mathcal{F}_{\mathsf{SSSumBucket}}$}\\
%     \\
%     \textbf{Inputs:}
%     \begin{itemize}
%     	\item $\mathcal{A}$ inputs shares $\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M$, and $X_A,V_A$;
%         \item $\mathcal{B}$ inputs shares $\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M$, and $X_B,V_B$;.
%     \end{itemize}
%     \textbf{Outputs:}
%     \begin{itemize}
%         \item $\mathcal{A}$ outputs $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$;
%         \item $\mathcal{B}$ outputs $\{\langle bg \rangle_B\}^{j,k},\{\langle bh \rangle_B\}^{j,k}$.
%     \end{itemize}
% \end{tcolorbox}
% \end{small}



% \paragraph{Security Proof} We show that \textbf{Algorithm 4} is secure against semi-honest adversaries. Formally, we have the following theorem.

\begin{theorem}
	Assume that $\mathcal{F}_{\mathsf{N2S}}$ and $\mathcal{F}_{\mathsf{SMUL}}$ are secure primitives. Then, \textbf{Algorithm \ref{alg:ssbuck}} (denoted as $\pi_4$) is secure against semi-honest adversaries in $\mathcal{F}_{\mathsf{N2S}},\mathcal{F}_{\mathsf{SMUL}}$-hybrid model, as in \textbf{Definition 4.1}.
\end{theorem}





\begin{proof}
	We begin by proving the correctness of \textbf{Algorithm \ref{alg:ssbuck}}, i.e., we prove that $\{\langle bg \rangle_A\}^{j,k} + \{\langle bg \rangle_B\}^{j,k}$ is equal to $\Sigma_i\{ s_{jk}\}^i\cdot \{ g \}^i$, and $\{\langle bh \rangle_A\}^{j,k}+\{\langle bh \rangle_B\}^{j,k}$ is equal to $\Sigma_i\{ s_{jk}\}^i\cdot \{ h \}^i$.
	
	From the protocol execution, we know that $\{\langle bg \rangle\}^{j,k}=\Sigma_i\{\langle s_{jk}\rangle\}^i\cdot \{\langle g \rangle\}^i$. We denote $\{\langle s_{jk}\rangle\}^i\cdot \{\langle g \rangle\}^i$ as $\{\langle p \rangle\}^i$, and according to functionality $\mathcal{F}_{\mathsf{SMUL}}$, we have $\{ s_{jk}\}^i\cdot \{ g \}^i=\{ p \}^i$ and $\{\langle p \rangle_A\}^i+\{\langle p \rangle_B\}^i=\{ p \}^i$.
	
	Therefore, we have the following equation,
	\begin{equation}
		\begin{aligned}\nonumber
		\{\langle bg \rangle_A\}^{j,k}+\{\langle bg \rangle_B\}^{j,k}&=\Sigma_i\{\langle p \rangle_A\}^i+\Sigma_i\{\langle p \rangle_B\}^i\\
		&=\Sigma_i\{ p \}^i\\
		&=\Sigma_i\{ s_{jk}\}^i\cdot \{ g \}^i
		\end{aligned}
	\end{equation}
		
	Similarly, we have $\{\langle bh \rangle_A\}^{j,k}+\{\langle bh \rangle_B\}^{j,k}=\Sigma_i\{ s_{jk}\}^i\cdot \{ h \}^i$.
	
	This proves the correctness of \textbf{Algorithm \ref{alg:ssbuck}}. 
	
	We now prove that we can construct two simulators $\mathcal{S}_{\mathcal{A}}$ and $\mathcal{S}_{\mathcal{B}}$, such that
	\begin{eqnarray}
		\begin{aligned}
		&\{\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa} \label{eqn5}\\
		&\cong\{\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa},
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}
		\begin{aligned}
		&\{\mathcal{S}_{\mathcal{B}}(1^\kappa,\textsf{Input}_B,\{\langle bg \rangle_B\}^{j,k},\{\langle bh \rangle_B\}^{j,k})\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa}\\
		&\cong\{\mathsf{view}_{\mathcal{B}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa}, 
		\end{aligned}
	\end{eqnarray}
	where $\mathsf{view}_{\mathcal{A}}^{\pi_4}$ and $\mathsf{view}_{\mathcal{B}}^{\pi_4}$ denote the views of $\mathcal{A}$ and $\mathcal{B}$, respectively, while $\textsf{Input}_A=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,X_A,V_A)$ and $\textsf{Input}_B=(\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M,X_B,V_B)$ denote the inputs of $\mathcal{A}$ and $\mathcal{B}$, respectively.
	
	We then prove the above equations for a corrupted $\mathcal{A}$.
	
	\paragraph{Corrupted $\mathcal{A}$} 
	%In this case, we construct a probabilistic polynomial-time simulator $\mathcal{S}_{\mathcal{A}}$ that, when given the security parameter $\kappa$, $\mathcal{A}$'s input $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M$, $X_A,V_A)$ and output $(\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$, can simulate the view of $\mathcal{A}$ in the protocol execution. To this end, we first analyze $\mathcal{A}$'s view $\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ in \textbf{Algorithm 4}. 
	In \textbf{Algorithm \ref{alg:ssbuck}}, the messages obtained by $\mathcal{A}$ are consisted of two parts. The first part is from the functionality $\mathcal{F}_{\mathsf{N2S}}$, i.e., $\{\langle s_{jk}\rangle_A\}^i$; the second part is from the functionality $\mathcal{F}_{\mathsf{SMUL}}$, i.e., $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$. 
	Therefore, $\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ consists of $\mathcal{A}$'s input $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A)$, the randomness $r_{\mathcal{A}}$, and the shares $(\{\langle s_{jk}\rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$.
	
	
	Given $\kappa$, $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A)$ and $(\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$, $\mathcal{S}_{\mathcal{A}}$ generates a simulation of $\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ as follows. 
	
	\begin{itemize}
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{N2S}}$, randomly generates $\{\langle s_{jk}'\rangle_A\}^i$, and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{N2S}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ outputs $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$ to simulate the functionality $\mathcal{F}_{\mathsf{SMUL}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ generates a simulation by outputting $(\{\langle g \rangle_A\}^i_M$, $\{\langle h \rangle_A\}^i_M$, $X_A$, $V_A$, $r_{\mathcal{A}}$,$\{\langle s_{jk}'\rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$.
	\end{itemize}
	
	Therefore, we have the following two equations:
	\begin{small}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathsf{view}_{\mathcal{A}}^{\pi_4}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A,r_{\mathcal{A}},\{\langle s_{jk}\rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}),
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A,r_{\mathcal{A}},\{\langle s_{jk}'\rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}). 
		\end{aligned}
	\end{eqnarray}
	\end{small}
		
	We note that the probability distributions of $\mathcal{A}$'s view and $\mathcal{S}_{\mathcal{A}}$'s output are identical.
	We thereby claim that Equation (\ref{eqn5}) holds.
	
	This completes the proof in the case of corrupted $\mathcal{A}$.
	Similarly, We can construct a simulator in the case of corrupted $\mathcal{B}$.
	In summary, \textbf{Algorithm \ref{alg:ssbuck}} securely computes $\mathcal{F}_{\mathsf{SSSumBucket}}$ against semi-honest adversaries in $\mathcal{F}_{\mathsf{N2S}},\mathcal{F}_{\mathsf{SMUL}}$-hybrid model.

	
\end{proof}







\subsection{SumBucket based on HESS}\label{proof-hess}

% \begin{small}
% \begin{tcolorbox}[colback=white,arc=0pt,outer arc=0pt,boxrule=0.7pt,enhanced,breakable,fontupper=\linespread{.8}\selectfont]
% \textbf{Functionality of SumBucket based on HESS $\mathcal{F}_{\mathsf{HESSSumBucket}}$}\\
%     \\
%     \textbf{Inputs:}
%     \begin{itemize}
%     	\item $\mathcal{A}$ inputs shares $\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M$, and $X_A,V_A$;
%         \item $\mathcal{B}$ inputs shares $\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M$, and $X_B,V_B$;.
%     \end{itemize}
%     \textbf{Outputs:}
%     \begin{itemize}
%         \item $\mathcal{A}$ outputs $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$;
%         \item $\mathcal{B}$ outputs $\{\langle bg \rangle_B\}^{j,k},\{\langle bh \rangle_B\}^{j,k}$.
%     \end{itemize}
% \end{tcolorbox}
% \end{small}



% \paragraph{Security Proof} We show that \textbf{Algorithm 5} is secure against semi-honest adversaries. Formally, we have the following theorem.

\begin{theorem}
	Assume that the additively homomorphic cryptosystem $\Pi=(\textsf{KeyGen}$, $ \textsf{Enc}$, $\textsf{Dec})$ is indistinguishable under chosen-plaintext attacks, $\mathcal{F}_{\mathsf{S2H}}$ and $\mathcal{F}_{\mathsf{H2S}}$ are secure primitives as mentioned before. Then, \textbf{Algorithm \ref{alg:hessbuck}} (denoted as $\pi_5$) is secure against semi-honest adversaries in $\mathcal{F}_{\mathsf{S2H}},\mathcal{F}_{\mathsf{H2S}}$-hybrid model, as in \textbf{Definition 4.1}.
\end{theorem}





\begin{proof}
	We begin by proving the correctness of \textbf{Algorithm \ref{alg:hessbuck}}, \ie we prove that $\{\langle bg \rangle_A\}^{j,k} + \{\langle bg \rangle_B\}^{j,k}$ is equal to $\Sigma_i\{ s_{jk}\}^i\cdot \{ g \}^i$, and $\{\langle bh \rangle_A\}^{j,k}+\{\langle bh \rangle_B\}^{j,k}$ is equal to $\Sigma_i\{ s_{jk}\}^i\cdot \{ h \}^i$.
	
	From the protocol execution, we know that the decryption of $\{[bg]_P\}^{j,k}$ is equal to $\{\langle bg \rangle_A\}^{j,k} + \{\langle bg \rangle_B\}^{j,k}$, where $\{[bg]_P\}^{j,k}=\Sigma_i\{s_{jk}\}^i\cdot\{[g]_{P}\}^i$. Therefore, we have $\{\langle bg \rangle_A\}^{j,k} + \{\langle bg \rangle_B\}^{j,k}=\Sigma_i\{ s_{jk}\}^i\cdot \{ g \}^i$. 
	Similarly, we have $\{\langle bh \rangle_A\}^{j,k}+\{\langle bh \rangle_B\}^{j,k}=\Sigma_i\{ s_{jk}\}^i\cdot \{ h \}^i$. This proves the correctness of \textbf{Algorithm \ref{alg:hessbuck}}. 
	
	In order to prove the security, we now construct the simulator $\mathcal{S}_{\mathcal{A}}$ and omit the symmetric construction for Corrupted $\mathcal{B}$.
	
	In \textbf{Algorithm \ref{alg:hessbuck}}, the messages obtained by $\mathcal{A}$ are consisted of two parts. The first part is from the functionality $\mathcal{F}_{\mathsf{S2H}}$, \ie $\{[g]_B\}^i,\{[h]_B\}^i$, and the second part is from the functionality $\mathcal{F}_{\mathsf{H2S}}$, \ie $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}$. 
	Therefore, $\mathsf{view}_{\mathcal{A}}^{\pi_5}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ consists of $\mathcal{A}$'s input $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A)$, the randomness $r_{\mathcal{A}}$, and the messages $(\{[g]_B\}^i,\{[h]_B\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$.
	
	
	Given $\kappa$, $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M, X_A,V_A)$ and $(\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$, $\mathcal{S}_{\mathcal{A}}$ generates a simulation as follows. 
	
	\begin{itemize}
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{S2H}}$, randomly selects $\{g'\}^i$ and $\{h'\}^i$, encrypts them using $\mathcal{B}$'s public key $PK_B$ and obtains $\{[g']_B\}^i,\{[h']_B\}^i$. It takes $\{[g']_B\}^i,\{[h']_B\}^i$ as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{S2H}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{H2S}}$, takes $\{\langle bg \rangle_A\}^{j,k}$ and $\{\langle bh \rangle_A\}^{j,k}$ as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{H2S}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ generates a simulation of $\mathsf{view}_{\mathcal{A}}^{\pi_5}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ by outputting $(\{\langle g \rangle_A\}^i_M$, $\{\langle h \rangle_A\}^i_M$, $X_A$, $V_A$, $r_{\mathcal{A}}$,$\{[g']_B\}^i,\{[h']_B\}^i,$ $\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})$.
	\end{itemize}
	
	Therefore, we have the following two equations:
	\begin{small}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathsf{view}_{\mathcal{A}}^{\pi_5}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,X_A,V_A,r_{\mathcal{A}},\{[g]_B\}^i,\{[h]_B\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}),
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k})\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,X_A,V_A,r_{\mathcal{A}},\{[g']_B\}^i,\{[h']_B\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k}). 
		\end{aligned}
	\end{eqnarray}
	\end{small}
		
	We note that as the additively homomorphic cryptosystem $\Pi$ is indistinguishable under chosen-plaintext attacks, the probability distributions of $\mathcal{A}$'s view and $\mathcal{S}_{\mathcal{A}}$'s output are computationally indistinguishable. 
	This completes the proof in the case of corrupted $\mathcal{A}$.
	
	In summary, \textbf{Algorithm \ref{alg:hessbuck}} securely computes $\mathcal{F}_{\mathsf{HESSSumBucket}}$ against semi-honest adversaries in $\mathcal{F}_{\mathsf{S2H}},\mathcal{F}_{\mathsf{H2S}}$-hybrid model.

	
\end{proof}







\subsection{Splitnode based on SS}\label{proof-splitnode}

% \begin{small}
% \begin{tcolorbox}[colback=white,arc=0pt,outer arc=0pt,boxrule=0.7pt,enhanced,breakable,fontupper=\linespread{.8}\selectfont]
% \textbf{Functionality of Splitnode based on SS $\mathcal{F}_{\mathsf{SSSplitNode}}$}\\
%     \\
%     \textbf{Inputs:}
%     \begin{itemize}
%     	\item $\mathcal{A}$ inputs shares $\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M$, and $X_A,V_A$;
%         \item $\mathcal{B}$ inputs shares $\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M,\{\langle s \rangle_B\}^i_M$, and $X_B,V_B$;.
%     \end{itemize}
%     \textbf{Outputs:}
%     \begin{itemize}
%         \item $\mathcal{A}$ outputs $\{\langle p \rangle_A\}^i_M$;
%         \item $\mathcal{B}$ outputs $\{\langle p \rangle_B\}^i_M$.
%     \end{itemize}
% \end{tcolorbox}
% \end{small}



% \paragraph{Security Proof} We show that \textbf{Algorithm 3} is secure against semi-honest adversaries. Formally, we have the following theorem.

\begin{theorem}
	Assume that $\mathcal{F}_{\mathsf{N2S}}$, $\mathcal{F}_{\mathsf{SMUL}}$, $\mathcal{F}_{\mathsf{SDIV}}$, $\mathcal{F}_{\mathsf{SSSumbucket}}$ and $\mathcal{F}_{\mathsf{SMAX}}$ are secure primitives as defined above. Then, \textbf{Algorithm \ref{alg:sssplit}} (denoted as $\pi_3$) is secure against semi-honest adversaries in $\mathcal{F}_{\mathsf{N2S}},\mathcal{F}_{\mathsf{SMUL}},$ $\mathcal{F}_{\mathsf{SDIV}},\mathcal{F}_{\mathsf{SSSumBucket}},\mathcal{F}_{\mathsf{SMAX}}$-hybrid model, as in \textbf{Definition 4.1}.
\end{theorem}





\begin{proof}
	We prove that we can construct two simulators $\mathcal{S}_{\mathcal{A}}$ and $\mathcal{S}_{\mathcal{B}}$, such that
	\begin{eqnarray}
		\begin{aligned}
		&\{\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle p \rangle_A\}^i_M)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa} \label{eqn6}\\
		&\cong\{\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa},
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}
		\begin{aligned}
		&\{\mathcal{S}_{\mathcal{B}}(1^\kappa,\textsf{Input}_B,\{\langle p \rangle_B\}^i_M)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa}\\
		&\cong\{\mathsf{view}_{\mathcal{B}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\}_{\textsf{Input}_A,\textsf{Input}_B,\kappa}, 
		\end{aligned}
	\end{eqnarray}
	where $\mathsf{view}_{\mathcal{A}}^{\pi_3}$ and $\mathsf{view}_{\mathcal{B}}^{\pi_3}$ denote the views of $\mathcal{A}$ and $\mathcal{B}$, respectively, while $\textsf{Input}_A=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M,X_A,V_A)$ and $\textsf{Input}_B=(\{\langle g \rangle_B\}^i_M,\{\langle h \rangle_B\}^i_M$, $\{\langle s \rangle_B\}^i_M,X_B,V_B)$ denote the inputs of $\mathcal{A}$ and $\mathcal{B}$, respectively. We prove the above equations for a corrupted $\mathcal{A}$ and omit similar construction for a corrupted $\mathcal{B}$.
	
	Without loss of generality, we assume that the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$ happens only once in \textbf{Algorithm \ref{alg:sssplit}}. That is, we assume that for the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$ at line 48 in \textbf{Algorithm \ref{alg:sssplit}}, $\mathcal{F}_{\mathsf{SSSplitNode}}$ directly runs lines 4-10 and returns $\{\langle y \rangle\}^i$ as $\{\langle p_l \rangle\}^i$. For the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$ at line 49 in \textbf{Algorithm \ref{alg:sssplit}}, $\mathcal{F}_{\mathsf{SSSplitNode}}$ directly runs lines 4-10 and returns $\{\langle y \rangle\}^i$ as $\{\langle p_r \rangle\}^i$. We note that this assumption is just for a simpler and clearer description of the security proof, and will not lead to any security issues during the simulation of corrupted $\mathcal{A}$ or corrupted $\mathcal{B}$.
	
	\paragraph{Corrupted $\mathcal{A}$}In \textbf{Algorithm \ref{alg:sssplit}}, the messages obtained by $\mathcal{A}$ are consisted of five parts. The first part is from the functionality $\mathcal{F}_{\mathsf{N2S}}$, \ie $\langle sg_{l}\rangle_A,\langle sh_{l}\rangle_A$ and $\{\langle s_l \rangle_A\}^i,\{\langle s_r \rangle_A\}^i$; the second part is from the functionality $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$, \ie $\langle cgain \rangle_A$, $\{\langle gain \rangle_A\}^{j,k}$, $\{\langle g_l \rangle_A\}^i,\{\langle h_l \rangle_A\}^i,\{\langle g_r \rangle_A\}^i,\{\langle h_r \rangle_A\}^i$, and the new shares $\{\langle s'_l \rangle_A\}^i,$ $\{\langle s'_r \rangle_A\}^i$; the third part is from the functionality $\mathcal{F}_{\mathsf{SSSumBucket}}$, \ie $\{\langle bg \rangle_A\}^{j,k},$ $\{\langle bh \rangle_A\}^{j,k}$; the forth part is from the functionality $\mathcal{F}_{\mathsf{SMAX}}$, \ie the indices $j_{best},k_{best}$; and the fifth part is from the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$. To be specific, the messages in this part are actually from the functionality $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$, \ie $node.\langle weight_1\rangle_A,$ $\{\langle p_l \rangle_A\}^i$ and $node.\langle weight_2\rangle_A, \{\langle p_r \rangle_A\}^i$. 
	
	Therefore, $\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ consists of $\mathcal{A}$'s input $(\{\langle g \rangle_A\}^i_M$, $\{\langle h \rangle_A\}^i_M$, $\{\langle s \rangle_A\}^i_M$, $X_A$, $V_A)$, the randomness $r_{\mathcal{A}}$, and the above mentioned indices and shares.
	
	
	Given $\kappa$, $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M, X_A,V_A)$ and $\{\langle p \rangle_A\}^i_M$, $\mathcal{S}_{\mathcal{A}}$ generates a simulation of $\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ as follows. 
	
	\begin{itemize}
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{N2S}}$, randomly generates $\langle sg'_{l}\rangle_A,\langle sh'_{l}\rangle_A$ and $\{\langle s''_l \rangle_A\}^i,\{\langle s''_r \rangle_A\}^i$, and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{N2S}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$, randomly generates $\langle cgain' \rangle_A$,
		$\{\langle gain' \rangle_A\}^{j,k}$,
		$\{\langle g'_l \rangle_A\}^i$,
		$\{\langle h'_l \rangle_A\}^i$,
		$\{\langle g'_r \rangle_A\}^i$,
		$\{\langle h'_r \rangle_A\}^i$, 
		$\{\langle s'''_l \rangle_A\}^i$,
		$\{\langle s'''_r \rangle_A\}^i$ and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{SSSumBucket}}$, randomly generates $\{\langle bg' \rangle_A\}^{j,k}$, $\{\langle bh' \rangle_A\}^{j,k}$, and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{SSSumBucket}}$.
		\item {$\mathcal{S}_{\mathcal{A}}$ simulates the functionality $\mathcal{F}_{\mathsf{SMAX}}$, randomly generates $j'_{best},k'_{best}$, and takes them as the output for $\mathcal{A}$ in $\mathcal{F}_{\mathsf{SMAX}}$.}
		\item $\mathcal{S}_{\mathcal{A}}$ simulates the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$. Specifically, during the recursion, $\mathcal{S}_{\mathcal{A}}$ needs to simulate the functionality $\mathcal{F}_{\mathsf{SMUL}}$ and $\mathcal{F}_{\mathsf{SDIV}}$ again as follows. It randomly generates $node.\langle weight'_1\rangle_A, node.\langle weight'_2\rangle_A, \{\langle p'_l \rangle_A\}^i$, computes $\{\langle p'_r \rangle_A\}^i=\{\langle p \rangle_A\}^i-\{\langle p'_l \rangle_A\}^i$, and takes them as the output for $\mathcal{A}$ in the recursion of $\mathcal{F}_{\mathsf{SSSplitNode}}$.
		\item $\mathcal{S}_{\mathcal{A}}$ generates a simulation of $\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)$ by outputting the inputs $(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M, X_A,V_A)$, the randomness $r_{\mathcal{A}}$, and all the simulated indices and shares above.
	\end{itemize}
	
	Therefore, we have the following two equations:
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathsf{view}_{\mathcal{A}}^{\pi_3}(\textsf{Input}_A,\textsf{Input}_B,\kappa)\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M, X_A,V_A,r_{\mathcal{A}},\langle sg_{l}\rangle_A,\langle sh_{l}\rangle_A,\{\langle s_l \rangle_A\}^i,\\
		&\{\langle s_r \rangle_A\}^i,\langle cgain \rangle_A,\{\langle gain \rangle_A\}^{j,k},\{\langle g_l \rangle_A\}^i,\{\langle h_l \rangle_A\}^i,\{\langle g_r \rangle_A\}^i,\\
		&\{\langle h_r \rangle_A\}^i,\{\langle s'_l \rangle_A\}^i,\{\langle s'_r \rangle_A\}^i,\{\langle bg \rangle_A\}^{j,k},\{\langle bh \rangle_A\}^{j,k},j_{best},k_{best},\\
		&node.\langle weight_1\rangle_A,node.\langle weight_2\rangle_A,\{\langle p_l \rangle_A\}^i,\{\langle p_r \rangle_A\}^i),
		\end{aligned}
	\end{eqnarray}
	\begin{eqnarray}\nonumber
		\begin{aligned}
		&\mathcal{S}_{\mathcal{A}}(1^\kappa,\textsf{Input}_A,\{\langle p \rangle_A\}^i_M)\\
		&=(\{\langle g \rangle_A\}^i_M,\{\langle h \rangle_A\}^i_M,\{\langle s \rangle_A\}^i_M, X_A,V_A,r_{\mathcal{A}},\langle sg'_{l}\rangle_A,\langle sh'_{l}\rangle_A,\{\langle s''_l \rangle_A\}^i,\\
		&\{\langle s''_r \rangle_A\}^i,\langle cgain' \rangle_A,\{\langle gain' \rangle_A\}^{j,k},\{\langle g'_l \rangle_A\}^i,\{\langle h'_l \rangle_A\}^i,\{\langle g'_r \rangle_A\}^i,\\
		&\{\langle h'_r \rangle_A\}^i,\{\langle s'''_l \rangle_A\}^i,\{\langle s'''_r \rangle_A\}^i,\{\langle bg' \rangle_A\}^{j,k},\{\langle bh' \rangle_A\}^{j,k},j'_{best},k'_{best},\\
		&node.\langle weight'_1\rangle_A, node.\langle weight'_2\rangle_A,\{\langle p'_l \rangle_A\}^i,\{\langle p'_r \rangle_A\}^i). 
		\end{aligned}
	\end{eqnarray}
	
	
	
		
	We note that the probability distributions of $\mathcal{A}$'s view and $\mathcal{S}_{\mathcal{A}}$'s output are identical.
	We thereby claim that Equation (\ref{eqn6}) holds. This completes the proof in the case of corrupted $\mathcal{A}$. 
	
	After similar construction for a corrupted $\mathcal{B}$, we conclude that \textbf{Algorithm \ref{alg:sssplit}} securely computes $\mathcal{F}_{\mathsf{SSSplitNode}}$ against semi-honest adversaries in $\mathcal{F}_{\mathsf{N2S}},\mathcal{F}_{\mathsf{SMUL}},\mathcal{F}_{\mathsf{SDIV}},\mathcal{F}_{\mathsf{SSSumBucket}},\mathcal{F}_{\mathsf{SMAX}}$-hybrid model.

\end{proof}
